Responsible AI for Earth Observation

The convergence of artificial intelligence (AI) and Earth observation (EO) technologies has brought geoscience and remote sensing into an era of unparalleled capabilities. AI's transformative impact on data analysis, particularly derived from EO platforms, holds great promise in addressing global challenges such as environmental monitoring, disaster response and climate change analysis. However, the rapid integration of AI necessitates a careful examination of the responsible dimensions inherent in its application within these domains. In this paper, we represent a pioneering effort to systematically define the intersection of AI and EO, with a central focus on responsible AI practices. Specifically, we identify several critical components guiding this exploration from both academia and industry perspectives within the EO field: AI and EO for social good, mitigating unfair biases, AI security in EO, geo-privacy and privacy-preserving measures, as well as maintaining scientific excellence, open data, and guiding AI usage based on ethical principles. Furthermore, the paper explores potential opportunities and emerging trends, providing valuable insights for future research endeavors.

==> 4-accountability.tex <==
\section{Accountability in AI4EO}
\label{sec:accountability}
%%%%%%%%%%%%%%%%%%%%%%%%%% Possible Outline %%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition of the related terminologies.
% Literature review for accountability in AI4EO.
% Future perspectives (potential research directions and trends).
  
% length: around 2-3 pages
% num of ref: around 20-40 refs
%%%%%%%%%%%%%%%%%%%%%%%%%% General Suggestions from Pedram %%%%%%%%%%%%%%%%%%%%%%%%%% 
% Problem definition (with key equations if needed), its role in RS, its categories (with a bird’s eye view), a few examples for each category, and some nice figures or tables

==> rspai_arxiv/0-introduction.tex <==
\section{Introduction}
In the evolving landscape of EO, the fusion of AI with Earth observation (EO) holds tremendous promise for unlocking insights into our planet's dynamics \cite{ghamisi2018new}. %GRS play important roles in comprehending and monitoring Earth's complex systems, from climate dynamics to land-use changes. 
Specifically, the integration of AI techniques for EO (AI4EO) significantly enhances our capacity to distill meaningful information from remotely sensed data \cite{zhu2017deep}, which became a substantial surge since 2020, as shown in Fig. \ref{fig:papers1}. %illustrates the escalating trend in AI4EO-related publications within key journals in GRS over the past decade, indicating a substantial surge since 2020. %The successful application of AI covers various aspects of EO missions, as outlined in Table \ref{table:ai4eo}. 
Nonetheless, the complex nature of Earth systems requires a thorough understanding of AI's inherent limitations and potential consequences, which necessitates the implementation of responsible AI practices in EO. This shapes the particular focus of this paper. 
%necessitates a well-informed approach to address issues such as bias, interpretability and unintended environmental and social impacts.
\begin{figure}
    \centering
    \includegraphics[scale=0.55]{figures/introduction/statistics.pdf}
    \caption{Number of AI4EO-related studies published in IEEE TGRS from 2014 to 2023. Data is collected from Google Scholar advanced search: keywords: ("machine learning" or "deep learning") and "remote sensing."}
    \label{fig:papers1}
\end{figure}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/introduction/respAI_devAI.pdf}
    \caption{Overview of the development of AI algorithms over the last decades. The focus of AI algorithms has shifted multiple times between being model-centric and data-centric. The blue part illustrates the historical development of AI concerning data and models, while the orange part reflects our beliefs in the EO community regarding current and future developments. The concept of responsible AI gained significant attention in the late 2010s and early 2020s. During this period, concerns about AI biases, fairness, transparency, and accountability began to receive increased attention.}
\label{fig:intro_devAI}
\end{figure*}
Fig. \ref{fig:intro_devAI} shows an overview of the development of AI algorithms over the last decades. The birth of AI as a distinct field is often attributed to a workshop held at Dartmouth College in the summer of 1956. The concept of responsible AI gained significant attention in the late 2010s and early 2020s, and with generative-adversarial approaches as one of the catalysts. During this period, concerns about AI biases, fairness, transparency and accountability began to gain prominence, with early influential works such as "Gender Shades" (2018) \cite{buolamwini2018gender} highlighting biases in facial recognition technologies. This era also saw the release of ethical guidelines like the IEEE's "Ethically Aligned Design" (2016) \cite{shahriari2017ieee} and the ACM's updated Code of Ethics (2018) \cite{gotterbarn2018acm}. In the early 2020s, regulatory efforts intensified with the European Commission's "Ethics Guidelines for Trustworthy AI" (2019) \cite{hleg2019ethics} and the OECD's AI Principles (2019) \cite{galindo2021overview}. Major tech companies like Google and Microsoft established dedicated responsible AI teams and initiatives. The concept of responsible AI continued to evolve, integrating into AI development pipelines and emphasizing both data quality and model innovation. Standardization efforts by organizations like ISO and educational initiatives further promoted responsible AI practices, addressing ethical considerations such as fairness, transparency, and bias mitigation. In our opinion, and as indicated by the light orange color in Fig. \ref{fig:intro_devAI}, we have transitioned from an era of singular focus on either model-centric or data-centric approaches to a new era characterized by balanced data-model approaches. This paradigm emphasizes both model innovation and data equally, exemplified by the rise of foundation models \cite{mai2023opportunities, hong2023spectralgpt}. Despite this shift, we believe responsible AI continues to play an increasingly important role in guiding the development and deployment of AI technologies.



%As artificial intelligence (AI) technologies increasingly invade Earth observation (EO) processes, influencing tasks such as predictive modeling for environmental changes, the need for a responsible AI framework becomes relevant. This technological evolution empowers AI systems to analyze vast datasets, providing insights into geological phenomena and environmental dynamics. However, the complexity of Earth systems demands a thorough understanding of AI's inherent limitations and potential consequences. The responsible development of AI in Earth observation requires an informed approach to issues such as bias, interpretability, and unintended environmental impacts.

From a technical perspective, the ambition of responsible AI goes beyond theoretical discussions and becomes a vital aspect of both research and application \cite{dignum2019responsible,9527092}. Therefore, this paper articulates the use of AI4EO with a particular focus on responsible practices, providing a comprehensive guide for the ethical design and deployment of AI in geospatial and environmental contexts. Considering the centrality of human decisions in shaping AI applications, we emphasize the incorporation of domain-specific values at every decision point. As discussed in this paper, responsible AI requires a systematic process to ensure that ethical considerations are incorporated into the body of AI4EO projects, from data collection to the interpretation of geospatial intuitions.

%\begin{table*}
%\caption{Representative Tasks in the geoscience and remote sensing field using Artificial Intelligence techniques}
%\label{table:ai4eo}
%\centering
%\begin{tabular}{cp{80mm}p{19mm}p{15mm}c}
%\specialrule{1pt}{0pt}{0pt}
%\textbf{Tasks}                        & \multicolumn{1}{c}{\textbf{Description}}                                                                                     & \textbf{AI Techniques}     & \textbf{Data Types}  & \textbf{References}  \\ \hline
%\textit{Low-level Vision Tasks}       &                                                                                                                              &                       &                      &                      \\ \vspace{0pt}
%Denoising                             & Mitigating the random noise contained in RS images.                                                               &   CNN                           & HSI                     &  \cite{shi2021hyperspectral}                    \\ \vspace{0pt}
%Panshapening                          & Creating a high-resolution color image with additional spectral information of the panchromatic band.                        &           CNN, TM                   &   HSI                   &    \cite{10103692}                  \\
%Cloud Removal                         & Eliminating clouds and cloud shadows that may impede the visibility of the Earth's surface.                                  &   CNN, GAN                      &   Optical, NIR                   & \cite{yu2022cloud}                     \\
%Destriping                            & Removing the stripe-like artifacts or patterns to enhance the clarity of the data.                                           &             RNN                 &     HSI                  &   \cite{li2023progressive}                   \\
%Super-resolution                      & Enhancing the spatial resolution of an RS image for improved analysis and interpretation.                                     &    DPM                          &   Optical                   &    \cite{xiao2023ediffsr}                  \\
%Adversarial Defense                   & Securing AI models against adversarial examples that markedly threaten the model's performance.                             & DPM            &    Optical, NIR                  &    \cite{yu2023universal}                  \\ \hline
%\textit{High-level Vision Tasks}      &                                                                                                                              &                        &                      &                      \\
%Land Cover Classification                     & Categorizing surface features in RS imagery to analyze and monitor Earth's surface.            &   CNN, TM                &   HSI, LiDAR, SAR                   & \cite{yao2023extended}                 \\
%Change detection                      & Identifying alterations in land cover and land use over time from multi-temporal RS imagery.                                 & SN, TM      &   Optical                   &    \cite{zhang2022multilevel}                  \\
%Object Detection                      & Identifying and locating multiple objects within an image or a video frame in RS imagery.                                     &  CNN, TM                      &        Optical              &   \cite{zhang2023efficient}                   \\
%Semantic Segmentation                 & Classifying and segmenting each pixel in an RS image into specific object classes.                                           &    CNN                    &   Optical, NIR                           &  \cite{xu2022consistency}                    \\ \hline
%\textit{NLP-related Tasks}            &                                                                                                                              &                        &                               &                      \\
%Image Captioning                      & Generating descriptive textual captions for the visual content.              &  CNN, LSTM                      &   Optical, Text                   &   \cite{cheng2022nwpu}                           \\
%Change Captioning                     & Generating descriptive textual captions to explain the variations from multi-temporal RS images.                      &  SN, RNN                      &     Optical, Text                            &   \cite{hoxha2022change}                   \\
%Visual Question Answering             & Understanding RS images and answering natural language questions related to the visual content. &    CNN, RNN                    &    Optical, Text                  &    \cite{lobry2020rsvqa}                              \\
%Text-to-image Generation              & Creating visually coherent and contextually relevant RS images from textual descriptions.                                    &   MHN                     &      Optical, Text                            &   \cite{xu2023txt2img}                   \\ \hline
%\textit{Environmental Monitoring}     &                                                     &                      \\
%Flood Detection          & Discerning alterations in water patterns to facilitate the precise identification and tracking of flooded regions.                                                             &  SN, CNN                      &    Optical, DEM                        &   \cite{yokoya2020breaking}                   \\
%Landslide Detection                   & Identifying potential landslide-prone areas using RS data to enhance early warning systems.     &FFSN                            & Optical, DEM   & \cite{liu2023feature} \\
%Wildfire Detection                    & Monitoring the occurrence of wildfires using RS imagery to support early detection and response efforts.                     & FCN   & Optical, MSI, SAR  & \cite{rashkovetsky2021wildfire} \\
%Deforestation Detection               & Monitoring the process of clearing or loss of forested areas using RS imagery to assess environmental impacts.               &    FCN                    &  Optical, NIR, MSI,                     &    \cite{torres2021deforestation}                  \\ \hline
%\textit{Advanced Learning Strategies} &                                                                                                                              &                        &                          &                      \\
%Weakly Supervised Learning            & Training with incomplete or imprecise labeling information with partially annotated data or noisy labels.                    &  CNN, TM                      &     Optical                      &    \cite{zhang2023weakly}                  \\
%Federated Learning                    & Training across decentralized edge devices or servers holding local data samples without exchanging them.                   &      DCNN, PM                  &     Optical                               &     \cite{zhang2023federated}                 \\
%Domain Adaptation                     & Improving the performance of a model on a target domain by leveraging knowledge gained from a different source domain.       &    CNN, DPRL                    &      Optical                               &   \cite{zhang2023cross}                  \\ \specialrule{1pt}{0pt}{0pt}
%\end{tabular}
%\end{table*}
\begin{figure}[!ht]
    \centering
    \includegraphics[scale=0.31]{figures/introduction/figures_respAI.pdf}
    \caption{Overview of the main building blocks of Responsible AI in EO: mitigating (unfair) biases, securing AI (defenses, uncertainty modeling, and explainability), preserving (geo)privacy, and addressing ethical concerns outline the considerations necessary for implementing responsible AI methodologies within the fields of EO. Social good presents the opportunities and goals related to how a responsible AI system can effectively be utilized to make a positive difference in people's lives.}
\label{fig:intro_overview}
\end{figure}
Fig. \ref{fig:intro_overview} shows the main considerations of responsible AI in EO, comprising the following five important aspects: %(1) mitigating unfair biases, (2) secure AI in EO, (3) geo-privacy, (4) ethical principles, and (5) AI4EO for social good. A brief introduction for each topic is given below:
\begin{itemize}
    \item \textit{Mitigating Unfair Bias (Section \ref{sec:unfair})} involves addressing and minimizing biases present in the algorithms and models used in AI4EO applications. Unfair bias can arise during many stages of the machine learning workflow, such as when the AI systems are trained on data that are not representative or when the data used for training contain inherent biases.
    \item \textit{AI Security in EO (Section \ref{sec:security})} focuses on implementing measures to increase the robustness, control of uncertainty and explainability of the AI systems and the data they process in the context of EO missions.
    \item \textit{Geo-Privacy and Privacy-Reserving Issues (Section \ref{sec:privacy})} aims to find a balance between leveraging the benefits of geospatial data for various EO applications while respecting and safeguarding individuals' privacy rights.
    \item \textit{Ethical Principles in AI4EO (Section \ref{sec:ethical})} introduces the guidelines and standards that govern the maintenance of scientific excellence, data availability and the guidance of AI usage in the context of EO research and applications.
    \item \textit{AI4EO for Social Good (Section \ref{sec:social})} refers to applying cutting-edge AI techniques to address and contribute positively to societal challenges and global issues. It aims to leverage advanced AI4EO technologies to find innovative solutions to pressing problems, promote sustainability, and enhance the overall wellbeing of communities.
\end{itemize}

The main contributions of this paper are as follows: Firstly, we present a pioneering and thorough review of the responsibility of AI research integrated with EO missions for the GRS society. Sections I-IV outline the considerations necessary for implementing responsible AI methodologies within the fields of EO, and Section V presents the opportunities and goals relating to how a responsible AI system can be effectively utilized for social good. This paper emphasizes that responsible AI is not merely a theoretical construct, but an imperative for advancing Earth observation and geosciences. By aligning technological advances with ethical considerations, this discourse aims to contribute to the ongoing dialogue surrounding the responsible and sustainable deployment of AI in the fields of EO and geosciences. Additionally, we dedicate a section (Section \ref{sec: business}) to showcasing the endeavors of private sectors in integrating responsible AI into their business models. This effort aims to foster innovation and sustainability within these sectors. Lastly, Section \ref{sec: conclusion} offers key remarks and actionable guidelines for researchers and practitioners to advance responsible AI practices in EO missions. This review is conducted from the perspectives of both academia and industry, as well as from both theoretical and practical points of view, to ensure a holistic view of the subject. %For every aspect, a theoretical introduction is given, accompanied by a detailed organization and description of various notable works, encompassing contributions from academic research as well as practical implementations from industry. The focus is on highlighting potential links with responsible AI for EO in each instance. 
%Furthermore, a perspective on the future outlook for each topic is presented to recognize the persistent challenges within the field of GRS. The comprehensive review is encapsulated with a focus on five potential research directions in AI4EO missions: benefits of AI4EO for society, fairness of AI models, securing AI models, data privacy and ethical guidance of AI4EO. Additionally, for each direction, we pinpoint potential opportunities and research trends to stimulate readers' interest in the domain of responsible AI.

%\begin{table}
%\caption{Main Abbreviations and Nomenclatures}
%\label{abbv}
%\begin{tabular}{cp{60mm}}
%\specialrule{1pt}{0pt}{0pt} % thicker line
%\textbf{Abbrev./Notation} & \textbf{Definition}                           \\ \hline
%AI                        & Artificial intelligence\\
%AI4EO                     & Artificial intelligence for earth observation \\
%BNN                       & Bayesian neural network\\
%CAM                       & Class activation mapping \\
%CNN                       & Convolutional neural network\\
%DCNN                      & Deep convolutional neural network \\
%DNN                       & Deep neural network\\
%DPM                       & Diffusion probabilistic model \\
%DPRL                      & Domain-aware progressive representation learning \\
%ECR-CAM                   & Encoder-classifier-reconstruction class activation mapping\\
%EO                        & Earth observation                             \\
%FFSN                      & Feature fusion semantic segmentation network\\
%FGSM & Fast gradient sign method\\
%IFGSM & Iterative fast gradient sign method\\
%LSTM & Long short-term Memory \\
%MIIDAOS-AI & AI-based multi-instrument inversion and data assimilation pre-processing %PM & Prototype Matching\\
%RS                        & Remote sensing \\
%SHAP                      & Shapely additive explanation \\
%SN                        & Siamese network \\
%TM                        & Transformer model \\
%XAI                       & Explainable artificial intelligence \\\hline
%$f$         & The classifier mapping of a neural network model \\
%$\alpha$    & The step size for iterative fast gradient sign method\\
%$\theta$    & A set of parameters in a neural network model \\
%$\theta^{*}$    & The optimized parameters of the trained model \\
%$\delta$    & The perturbation in adversarial examples \\
%$\delta^{*}$    & The optimal adversarial perturbation \\
%$x$ & A sample from the image space \\
%$y$ & The corresponding label of $x$ \\
%$\nabla$ & The gradient function \\
%$\mathcal{D}$ & The training dataset\\
%$K$ & Number \\
%$\mathcal{L}$ & The loss function\\
%$\mathcal{X}$ & The image space\\
%$\mathcal{Y}$ & The label space\\
%$\mathbf{sign}(\cdot)$ & Signum function\\
%\specialrule{1pt}{0pt}{0pt} % thicker line
%\end{tabular}
%\end{table}

%Table \ref{abbv} provides the main abbreviations and nomenclatures used in this paper. 
%The rest of this paper is organized as follows. 
%Section \ref{sec:social} introduces the advantages of AI along with the EO techniques for social good. Section \ref{sec:unfair} reviews the approaches in the EO applications that aim to mitigate the problem of unfair bias. Section \ref{sec:security} reviews the security hazards and corresponding solutions of the AI techniques in the geoscience and RS field. %Section \ref{sec:accountability} describes the accountability in the development, deployment, and use of AI technologies in the context of Earth observation. 
%Section \ref{sec:privacy} focuses on concerns about model and data privacy, and the associated protection measures that arise in AI4EO applications. Section \ref{sec:ethical} discusses the ethical issues that arise when developing and utilizing AI algorithms in EO missions. \textcolor{blue}{Sections I-IV outline the constraints and crucial considerations necessary for implementing responsible AI methodologies within the fields of remote sensing and geosciences. Section V presents the opportunities and goals for how a responsible AI system can be effectively utilized for social good.}


==> rspai_arxiv/1-social-good.tex <==
\section{AI\&EO for Social Good}
\label{sec:social}

In this section, we build upon the discussions in Section \ref{sec:ethical} regarding the use of AI4EO for social good, which involves applying AI technologies to address and solve social, economic and environmental challenges such as healthcare, education, environmental sustainability, poverty alleviation and disaster response. By leveraging AI technologies and the ethical considerations mentioned in the previous sections, these initiatives seek to improve outcomes and make a positive difference in people's lives, which is the ultimate goal of responsible AI.

Although the applications of AI4EO for social good are extensive \citep{persello2022deep,burke2021using}, we focus here primarily on understanding disaster risks and evaluating their impacts through several key examples crucial for effective disaster management and financing strategies \cite{SocialGood_IPCC22,SocialGood_IPCC21,SocialGood_AdaptPathways}. Robust frameworks are necessary for investing in projects that enhance resilience to climate change and its associated disasters. AI, leveraging integrated EO data, can significantly contribute to building these frameworks by analyzing such data through innovative computational methods \cite{SocialGood_AI,SocialGood_IPCC22,SocialGood_IPCC21}. %This can improve decision-making processes and aid adaptation efforts by considering the constantly evolving elements of climate \cite{SocialGood_AdaptPathways}. To address the current and future impact of climate change on human welfare and the environment, several adaptation and mitigation strategies have been implemented at international levels, such as the EU Green Deal, Singapore Green Plan, and the US Inflation Reduction Act. 
However, it is also crucial to implement policies and decisions at the local level, as the impacts of climate change vary over time and across different regions \cite{SocialGood_IPCC22,SocialGood_ECMWF,SocialGood_GreenDeal,SocialGood_SG_GreenPlan,SocialGood_USlegisl}.
%%%%%%%%%%%%%%%%%%%%%%%%%% Possible Outline %%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition of the related terminologies.
% Literature review for AI&EO for social good in remote sensing.
% Future perspectives (potential research directions and trends).

% length: around 2 pages
%%%%%%%%%%%%%%%%%%%%%%%%%% General Suggestions from Pedram %%%%%%%%%%%%%%%%%%%%%%%%%% 
% Problem definition (with key equations if needed), its role in RS, its categories (with a bird’s eye view), a few examples for each category, and some nice figures or tables

%A thorough understanding and assessment of natural and human-caused disaster risks, and evaluation of the impacts of disasters that occur, is essential for building robust frameworks for disaster management and financing strategies. Robust frameworks are vital for citizens, local authorities, and businesses to invest in projects that increase resilience to climate change, in particular, to prevent and mitigate the effects of climate-driven disasters \cite{SocialGood_IPCC22,SocialGood_IPCC21,SocialGood_AdaptPathways}.

%AI used on integrated Earth Observation data can play a key role in building robust frameworks. Investigating remote sensing data by means of innovative computational methods can lead to a greater understanding of the complex phenomena induced by climate change, and can lead to better-informed decision-making processes \cite{SocialGood_IPCC22,SocialGood_IPCC21,SocialGood_AI}. Using AI to consider the elements of climate that are constantly evolving can aid adaptation efforts and facilitate timely policy change  \cite{SocialGood_AI,SocialGood_IPCC22,SocialGood_AdaptPathways}.

%To address the current and future impact of climate change on human welfare and the environment, several adaptation and mitigation strategies were implemented at international levels (e.g., EU Green Deal, Singapore Green Plan, and US Inflation Reduction Act). However, it is also crucial to address the implementation of policies and decisions at the local level, as the impacts of climate change vary over time and across space \cite{SocialGood_IPCC22,SocialGood_ECMWF,SocialGood_GreenDeal,SocialGood_SG_GreenPlan,SocialGood_USlegisl}. 

Understanding disaster risks and evaluating their impacts are crucial for effective disaster management and financing strategies \cite{SocialGood_IPCC22,SocialGood_IPCC21,SocialGood_AdaptPathways}. Robust frameworks are necessary for investing in projects that enhance resilience to climate change and its associated disasters. AI leveraging integrated EO data can contribute significantly to building these frameworks by analyzing such data through innovative computational methods \cite{SocialGood_AI,SocialGood_IPCC22,SocialGood_IPCC21}. % This can improve decision-making processes and aid adaptation efforts by considering the constantly evolving elements of climate \cite{SocialGood_AdaptPathways}. To address the current and future impact of climate change on human welfare and the environment, several adaptation and mitigation strategies have been implemented at international levels (e.g., EU Green Deal, Singapore Green Plan, and US Inflation Reduction Act). 
 Moreover, it is also crucial to address the implementation of policies and decisions at the local level, as the impacts of climate change vary over time and across space \cite{SocialGood_IPCC22,SocialGood_ECMWF,SocialGood_GreenDeal,SocialGood_SG_GreenPlan,SocialGood_USlegisl}. 
%For example, increasing temperatures in Europe lead to increased evapotranspiration processes which, in turn, might increase the occurrence of floods in Germany, while water shortages could become more frequent in Italy. Simultaneously, Portugal, France, and Greece could be affected by a higher occurrence of wildfires caused by the same processes. Thus, it is crucial to enable each region to be prepared and ready to implement specific contingency plans based on local changes to environmental events characterized by changes in atmospheric and oceanographic variables \cite{SocialGood_ECMWF,SocialGood_ESA,SocialGood_IPCC22,SocialGood_GreenDeal}. The water cycle is also affected by global warming. This leads to the need for increasing irrigation to ensure vegetation health for food and biodiversity security. However, it has been demonstrated that increased irrigation can be connected to the increased occurrence of natural hazards, even at considerable distances. For example, examining North America closely, irrigation patterns in the Central Valley, High Plains and the Mississippi River Valley impact precipitation in the Colorado River, USA Midwest, and Southeast, respectively \cite{SocialGood_Irrig1,SocialGood_Irrig2,SocialGood_Irrig3,SocialGood_Irrig4}. 
For example, rising temperatures in Europe can intensify evapotranspiration, potentially causing more floods in Germany and water shortages in Italy. Meanwhile, Portugal, France, and Greece may face increased wildfires due to similar processes %Thus, it is vital to equip each region with tailored contingency plans based on local environmental changes driven by shifts in atmospheric and oceanographic variables 
\cite{SocialGood_ECMWF,SocialGood_ESA,SocialGood_IPCC22,SocialGood_GreenDeal}. Global warming also impacts the water cycle, necessitating increased irrigation for vegetation health and food security. This can heighten the occurrence of natural hazards, even across significant distances. For example, irrigation in North America's Central Valley, High Plains, and Mississippi River Valley affects precipitation in regions like the Colorado River, USA Midwest, and Southeast, respectively \cite{SocialGood_Irrig1,SocialGood_Irrig2,SocialGood_Irrig3,SocialGood_Irrig4}.


The above instances emphasize the diverse impacts of climate change on different regions, even at relatively close range. Thus, it is crucial to enable each region to be prepared and ready to implement specific contingency plans based on local changes to environmental events characterized by changes in atmospheric and oceanographic variables \cite{SocialGood_AdaptPathways,SocialGood_ECMWF,SocialGood_GreenDeal,SocialGood_IPCC22}. 
It is also worth noting that these changes might affect the socio-economic fabric of diverse biogeographic regions, thereby influencing the stability and security of human welfare and demographic fluxes \citep{SocialGood_AdaptPathways,SocialGood_ECMWF,SocialGood_GreenDeal,SocialGood_IPCC21,SocialGood_IPCC22,SocialGood_SG_GreenPlan}. 
It is, therefore, paramount for AI to provide a deep understanding of EO data so that decision- and policymakers are enabled to implement climate change adaptation and mitigation strategies. These strategies affect investments and solutions that citizens, local authorities, and businesses can undertake. Additionally, it implies the ability to engage stakeholders and public opinion to gain societal consensus %This means that economic recovery and societal readiness should be considered by adaptation and mitigation strategies so that all parts of the communities are included 
\cite{SocialGood_ECMWF,SocialGood_ESA,SocialGood_AI,SocialGood_GreenDeal}. 

%=====================================
%\subsection{Earth Observation Data}

%Retrieving information from EO, which allow for a global view of multiple atmospheric and oceanographic variables, as well as information on land, biosphere and cryosphere, with steady acquisitions across time, can provide a valuable tool that governments and local communities can use to create regional regulatory strategies to cope with climate change and keep track of the challenges imposed by climate transformation \cite{SocialGood_ESA,SocialGood_AI,SocialGood_GreenDeal,SocialGood_IPCC22}.


%The current efforts put in place by international organizations towards the development of innovative technologies for EO support the implementation of effective policies for climate change adaptation and mitigation, taking advantage of insights from environmental data analysis based on EO. For example, the European Space Agency (ESA) satellite fleet has become a benchmark for environmental data collection and in-depth analysis following a consistent and steady investment (22.2$\%$) of the ESA budget in the EO programme. %Moreover, the discovery and extraction of patterns in large datasets are enabled by multimodal remote sensing, which involves investigating arrays of data at differing spatial, spectral, temporal and radiometric resolutions. This approach allows for a better understanding of physical phenomena on the ground by combining data from multiple platforms. \cite{SocialGood_ESA,SocialGood_GreenDeal,SocialGood_ECMWF}.

%The open datasets provided by satellite constellations allow researchers and decision-makers to obtain a global picture of factors influencing our climate, such as temperature, vegetation, water quantity and quality. This enables public administrations, citizens and businesses to be better prepared for extreme events and crises. Moreover, better monitoring and more precise characterization of critical environmental parameters achieved by reliable AI-based EO analysis, such as biophysical assessment, natural resources use, potentials and limits for water quality examination, atmospheric pollution, and monitoring of natural disasters and catastrophic events, offer the opportunity to develop adequate solutions to critical factors and vulnerabilities \cite{SocialGood_ESA,SocialGood_GreenDeal,SocialGood_ECMWF,SocialGood_IPCC22,SocialGood_IPCC21}. 
 
To provide concrete examples of the actual impact and possibilities unlocked by the appropriate use of AI in decision-making processes, we present two instances of operational scenarios that would benefit greatly from a deep understanding of Earth processes to enhance human welfare and improve communities' wellbeing.


%\subsection{Air Pollution Monitoring} 

%Air pollution (e.g., Fig. \ref{}) is formally defined as the contamination of indoor and outdoor air through chemical, physical or biological agents that are harmful to humans, animals, vegetation, and other organisms \cite{SocialGood_Air_WHO_1}. The main sources of air pollution can be human-caused (e.g., motor vehicles, industrial facilities) or natural (e.g., volcanic eruptions, windblown dust). Human welfare and the environment are severely affected by air pollution, given the wide scale of this phenomenon and its dispersed nature. Air pollution contributes directly to global warming, hence posing risks to the global climate. Additionally, epidemiological studies over the past decades have shown the health risks that air pollution might induce, including heart disease, lung cancer, diabetes, and respiratory infections. Moreover, air pollution has been identified as a main factor in approximately seven million premature deaths annually \cite{SocialGood_Air_WHO_1,diabetes1}. 

%The implications and effects of air pollution on individuals and communities have a deep and far-reaching impact that deserves to be explored and characterized. Indeed, the negative effects of air pollution on society can be limited, controlled, and reduced by a deeper understanding of this phenomenon. This characterization implies \cite{SocialGood_AI,SocialGood_AdaptPathways,SocialGood_Air_WHO_1,diabetes1,capacity}:
%\begin{itemize}
%    \item Inferring correlations and trends between regions of air pollution to raise awareness of linked factors and causes of the overall issue.
%    \item Gaps in data are common due to underdeveloped technology or faulty data synchronization. Deriving a complete set of air pollution records drawn from the data from a dataset with gaps can increase the reliability and quality of any conclusions.
%    \item Identifying similarities and differences between pollutant regions and species can increase the accuracy of any obtainable results and strengthen overall understanding of the causes and effects of air pollution.
%\end{itemize}
%To achieve these objectives, the characterization of air pollution trends is fostered by exploiting the increasing dimensionality of environmental data, mainly caused by advances in remote sensing technology. This increase comes with the variety and quantity of sensors in use, facilitated by advanced artificial intelligence techniques \cite{capacity,diabetes1,fluid_arxiv,SocialGood_Air_AGU23}. 
%Indeed, a concise and representative global view of the system is key to identifying the interdependencies between different data points, thereby understanding the causes and effects of the measured air pollution trends.

%Among the recent developments in air pollution studies, graph-based data analysis investigating remote sensing records has shown very promising results \cite{fluid_ICASSP23,fluid_arxiv,SocialGood_Air_AGU23,Iain_arxiv}. In this approach, graph nodes represent the locations of air pollution monitoring stations, characterized by records collected in environmental data (e.g., humidity, temperature), as well as measurements of multiple species of pollutants (i.e., PM2.5, PM10, NO2, O3). Additionally, socio-economic and administrative records (e.g., land use, land cover, road traffic) are considered to explore and understand the implications of air pollution on the societal, health, and financial aspects of communities. Processing the information in this architecture through nonlinear optimization schemes enables the management and overcoming of mismatches and undesired effects in temporal and spatial resolutions of measurements. This allows learning the type, relevance, and properties of connections linking the nodes \cite{SocialGood_Air_AGU23,fluid_ICASSP23,Iain_arxiv}.

%The above architecture enables the retrieval of information on the causes and effects of multispecies air pollution trends. Additionally, investigating the structure of the data space induced by the graph generated by the air pollution data (i.e., the degree of similarity and interplay of the diverse factors) can produce a deep understanding of the properties of anthropogenic and environmental processes that led to them. The validity of this approach is demonstrated by cross-validating records acquired by satellites, ground stations, and climatic projections. This leads to deriving valuable information for the characterization of air pollution processes which, in turn, results in relevant information that local administrations and decision-makers can use to reduce the impact of this phenomenon on their communities \cite{SocialGood_Air_AGU23,Iain_arxiv,fluid_arxiv}.


%\begin{figure}[htb]
%	\centering
%	\includegraphics[width=1\columnwidth]{figures/ai_social_good/GRSM24_figure_LAQN_red.eps}
%	\caption{Identification of areas of similar air pollution properties in the London greater area by means of the procedure in \cite{SocialGood_Air_AGU23}.}
%	\label{SocialGood_AirPollution}
%\end{figure}



%\subsection{Sea Level Rise}

%The last decades have been characterized by a global sea-level rise at an unprecedented rate caused by climate change \cite{SocialGood_NOAA}. Sea-level rise presents an increasing risk to coastal regions, especially those that are low-lying, densely populated, and have a large number of important energy, communication, and residential infrastructures \cite{SocialGood_GreenDeal,SocialGood_IPCC21,SocialGood_IPCC22,SocialGood_SG_GreenPlan}. Therefore, it is important to find efficient and effective ways to mitigate the effects of sea-level rise in these areas and implement adaptive measures. However, studying these immediate effects and consequences on coastal regions and the communities dwelling in these areas might be cumbersome, since the interplay and number of interactions among environmental factors at a global scale is very high, hence jeopardizing the reliability and robustness of the proposed analysis \cite{SocialGood_Horton,SocialGood_NOAA}.

%Taking advantage of technological advances in AI strategies and the global coverage of sea level rise acquired by EO platforms is crucial to increasing our understanding of sea level rise processes \cite{SocialGood_ESA,SocialGood_ECMWF}. In fact, it is possible to draw inspiration from recent achievements in diverse data science domains to enhance the capacity to retrieve information on the impact and effects of sea level rise \cite{SocialGood_SocialOcean2,SocialGood_GraphProp,SocialGood_SocialOcean}. It is possible to model the interplay of changes in sea-level processes at different regional scales as "connections" across ocean regions \cite{SocialGood_SocialOcean}. Thus, it is feasible to derive a graph representation capable of incorporating the interplays measured by processes across diverse regions in the sea, forming a "social network of the ocean." The mathematical structure provided by graph-based data analysis enables the modeling of pairwise relations and exploration of complex relationships between various geographical locations in the context of sea-level rise, facilitating the design of targeted solutions to tackle this issue \cite{SocialGood_SocialOcean}.

%It is paramount to include in the graph representation several types of datasets characterizing sea-level processes across the world \cite{SocialGood_SocialOcean,SocialGood_SocialOcean2}. Multimodal EO \cite{capacity} is crucial because remote sensing platforms can provide global coverage of multiple sea-level indicators as well as digital elevation models of coastal regions. Simultaneously, investigating such massive and heterogeneous datasets requires the development of novel methods capable of managing the high degree of nonlinearity induced by such groups of records. In fact, working with multiple sources of data implies the presence of both temporal and static data, and a mismatch in resolution and scale across datasets. Therefore, it is important to develop AI architectures capable of reconciling the differences in the datasets so that they can be used together, and information can be reliably extracted \cite{SocialGood_NOAA,SocialGood_ECMWF}.
 
%Using nonlinear graph-based data analysis strategies, it is possible to derive important properties of the sea-level rise dynamics graph \cite{SocialGood_SocialOcean}. In fact, quantifying the centrality of the graph nodes allows for the calculation of the relevance of various coastal regions to identify locations that are more "influential" at sea (according to the previously mentioned analogy to social network data analysis) \cite{SocialGood_SocialOcean2,SocialGood_GraphProp}. This results in the quantification of the impact of perturbations to sea level, as nodes that are more central in the graph representation can be associated with locations where the impact of sea level rise is most felt and measured. Consequently, studying the interplay across these nodes and how changes in sea-level rise processes can propagate across the graph (by means of random walk-inspired signal propagation) leads to understanding the effects of climate perturbations and especially extreme events across the globe. This information is crucial for sea-level rise adaptation and mitigation since it enables the characterization of how the occurrence of extreme events (e.g., typhoons, tsunamis) under diverse climate scenarios might affect coastal regions \cite{SocialGood_IPCC22,SocialGood_ECMWF,SocialGood_NOAA,SocialGood_SG_GreenPlan}. This paves the way to make coastal communities and governments able to take advantage of accurate and reliable information on the possible impact of extreme events, hence allowing the implementation of timely measures for emergency preparedness and damage assessment and prevention.

 
%\begin{figure}[htb]
%	\centering
%	\includegraphics[width=1\columnwidth]{figures/ai_social_good/GRSM24_figure_ocean.eps}
%	\caption{Simulation of the impact of a storm surge in Southern Ocean (Antarctica) quantifying the areas that could be more affected in a red color scale \cite{SocialGood_SocialOcean}.}
%	\label{SocialGood_SeaLevelRise}
%\end{figure}



\subsection{Early Warning Systems for Mass Movements}

One of the most severe effects of climate change is the increased occurrence of catastrophic events caused by mass movements. This affects human welfare and results in huge economic losses. As such, the development of early warning systems (EWSs) is crucial to the everyday decisions of local governments and communities, and exemplify Responsible AI by prioritizing human safety and equity through timely alerts and accessible technology \cite{SocialGood_AdaptPathways,SocialGood_ECMWF,SocialGood_GreenDeal,SocialGood_IPCC21,SocialGood_IPCC22}. 

Historically, the main objective of EWSs has been to quantify the degree of immediate danger that every human settlement in each region of interest is exposed to (see, \cite{azarafza2021deep,SocialGood_EWS1,SocialGood_EWS2,SocialGood_EWS3}). In fact, state-of-the-art EWSs used in operational pipelines are based on the analysis of data and measurements at the regional level, which are then aggregated to avoid issues related to the irregularity of the temporal and spatial scale at which each record can be acquired. In this way, state-of-the-art EWSs are prone to highly sensitive and coarse classifications and predictions, potentially leading to a poor perception of risk and inadequate local management plans. Moreover, the classic structure of operational EWSs does not account for cascading effects affecting local communities at social and economic levels. For example, state-of-the-art EWSs for mass movements do not consider a town that can be cut off from transportation and communication systems because of landslides blocking the roads around it as relevant for early warning \cite{SocialGood_EWS3}. 

AI4EO can be a game-changer in this arena \cite{SocialGood_ESA,SocialGood_ECMWF}. Recent studies \cite{SocialGood_EWS_AGU23} have shown the improvement to state-of-the-art EWSs' capacity provided by analysis of the environmental (hydrological and geological) characteristics of mass movements derived from remote sensing platforms and the connectivity information of formal settlements and road network data in terms of graph structures. This architecture allows us to study the interaction of the probabilistic mass movement susceptibility (derived from the environmental properties by means of a supervised ensemble graph neural network) on the graph representing the communication network (that could involve roads, electricity grids, water pipelines) connecting the formal settlements. Investigating this structure by graph-based methods (e.g., spectral clustering) results in the derivation of indices to quantify the probability of each human settlement to be directly or indirectly affected by mass movements (i.e., the probability to be hit by a mass movement event - such as a landslide - or the probability to be isolated as a result of mass movements affecting their surroundings) \cite{SocialGood_EWS_AGU23}. This approach has the capacity to pave the way for measures and policies for adaptation and mitigation through a new holistic graphical perspective to assess various large-scale geospatial datasets of risk elements such as exposure, vulnerability and hazard. In particular, it has been shown that this strategy can deliver robust and reliable outcomes for hindcasting and forecasting of the impact of mass movements at different scales (local, regional, and national), able to explore long temporal trends (e.g., over 68,000 incidents of reported mass movements since 1957) and accurately identify the critical factors for climate change-induced mass movements \cite{SocialGood_EWS_AGU23}.




\begin{figure}[htb]
	\centering
	\includegraphics[width=.5\columnwidth]{figures/ai_social_good/GRSM24_figure_EWS.eps}
	\caption{Estimation of mass movements susceptibility index across the Norwegian territory by means of the architecture proposed in \cite{SocialGood_EWS_AGU23}.}
	\label{SocialGood_EWS}
\end{figure}

\subsection{Climate Teleconnections}

One of the most important open challenges in environmental monitoring and climate change studies is represented by the analysis of climate teleconnections, that is, the investigation of the interplay between weather phenomena at widely separated locations on Earth. This implies the study of climate patterns that span thousands of kilometers. Examples of teleconnection phenomena include shifts of atmospheric mass and/or pressure back and forth between two distant locations, where changes in atmospheric pressure in one location lead to corresponding changes in pressure in another location far away \cite{SocialGood_Telecon7,SocialGood_Telecon8,SocialGood_Telecon9}. Therefore, responsible AI-driven insights are crucial for informing global climate strategies and policies to ensure that all communities benefit equitably.

The water cycle is one of the primary drivers of climate teleconnections worldwide. In this respect, the three world poles (i.e., Arctic, Antarctic, high mountain Asia (HMA)) play a key role in influencing global weather patterns through their impact on teleconnections \cite{SocialGood_Telecon1,SocialGood_Telecon2,SocialGood_Telecon3,SocialGood_Telecon4}. Specifically, the weather and climate of HMA and the surrounding region have been demonstrated to be influenced by global modes of variability (MoV), which are fluctuations of atmospheric and oceanographic variables (e.g., sea surface temperature, rainfall, surface pressure, wind speed) caused by the continuous exchange of mass, momentum and energy on all timescales between Earth’s atmosphere, oceans, cryosphere and continental hydrology. For example, the planetary-scale Rossby-wave propagation that causes the intra-seasonal variability over central Asia and the northern part of India has been demonstrated to be affected by the Eurasian teleconnection. Also well-known is the interplay and impact on HMA climate variations of the Indian Ocean Dipole (IOD) and El Niño Southern Oscillation (Nino34), North Atlantic Oscillation (NAO), the Central Indian Ocean mode, and the boreal summer intraseasonal oscillation. However, a thorough understanding of the historical behavior of global MoV and its influence on weather patterns within the HMA has not yet been derived \cite{SocialGood_Telecon1,SocialGood_Telecon2,SocialGood_Telecon3,SocialGood_Telecon4,SocialGood_Telecon5,SocialGood_Telecon6,SocialGood_Telecon8,SocialGood_Telecon7}.

The use of advanced technologies for machine learning, relying on records acquired by EO platforms, plays a key role \cite{SocialGood_Telecon9,SocialGood_Telecon7}. In fact, as remote sensors can acquire properties of the previously mentioned environmental variables with precision at a global scale, they enable the investigation of MoVs that drive climate teleconnections worldwide. In particular, when considering HMA, the integration of remote sensing data with hydrometeorological climate variables (e.g., geopotential height at 250 hPa (z250), 2-m air temperature (T2M), total precipitation (PRECTOT), and fractional snow cover area (fSCA)) leads to a comprehensive exploration of the interactions across several MoVs over HMA (e.g., the Eurasian teleconnection, the IOD, the NAO and the Nino34). This results in the quantification of correlations and cause/effect scenarios across MoVs and climate variables, as well as the predictability of weather and climate patterns of the variables of interest, so that proper planning of resources and policies to address and adapt to climate change can be put in place \cite{SocialGood_ESA,SocialGood_AdaptPathways,SocialGood_GreenDeal,SocialGood_IPCC22,SocialGood_IPCC21,SocialGood_SG_GreenPlan,SocialGood_ECMWF}. %Also, this allows us to obtain a thorough overview of the implications of the identified relationships at weather, seasonal, or climate timescales, thus, quantifying the effect of climate teleconnections on socioeconomic factors. Finally, identifying and modeling the interplay across MoVs can lead to the proper characterization of the occurrence of extreme events and the understanding of their causes, to support prevention and disaster impact reduction for the benefit of communities and stakeholders \cite{SocialGood_Telecon9,SocialGood_Telecon7,Iain_CIKM}.




==> rspai_arxiv/2-unfair-bias.tex <==
\section{Mitigating (Unfair) Bias}
\label{sec:unfair}
%%%%%%%%%%%%%%%%%%%%%%%%%% Possible Outline %%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition of the related terminologies.
% Literature review for mitigating unfair bias in remote sensing.
% Future perspectives (potential research directions and trends).

% length: around 2 pages
%%%%%%%%%%%%%%%%%%%%%%%%%% General Suggestions from Pedram %%%%%%%%%%%%%%%%%%%%%%%%%% 
% Problem definition (with key equations if needed), its role in RS, its categories (with a bird’s eye view), a few examples for each category, and some nice figures or tables

Biases are inherent in all machine learning algorithms. Indeed, courses on machine learning often start with the bias-variance tradeoff, where biases occur when a model is under-fitting and are reduced as model complexity increases. This reduction of model bias is paired with an increase in variance errors as the complexity of the model overfits on variances in training data which are not representative of the target class in general. "Bias" is also a term linked to the systematic errors of an algorithm or dataset. Despite the concept of bias being inherent to machine learning, nowadays there is much concern for biases present in algorithms. Indeed, a review of Responsible AI guidelines and recommendations concluded that the principles of fairness and non-discrimination should be included in all AI guidance documents \cite{fjeld2020principled}. The difference here is that society is particularly concerned about "unfair" biases captured in machine learning algorithms. Generally speaking, this arises where the model systematically produces differing outcomes for specific subgroups of a class in a way that causes societal concern that is "unfair". The unfairness of the model is, therefore, contextual and closely linked to the values of a society. Friedman and Nissenbaum \cite{friedman1996bias}, thus, refer to biases that cause unfair and systematic discrimination of individuals or sub-groups of the population. Preventing discriminatory behavior is also considered to be the responsibility of the developer and user of AI algorithms. The UNESCO Recommendations on Ethical AI adopted by all member states in 2021 states: "AI actors should make all reasonable efforts to minimize and avoid reinforcing or perpetuating discriminatory or biased applications and outcomes throughout the life cycle of the AI system to ensure fairness of such systems" \cite{unesco2021recommendation}. Similarly, the European Commission is drafting an AI Act that incorporates a requirement to consider and report potential biases \cite{euaiact2021}. Understanding how to audit AI workflows for biases and how to mitigate them are expected to be two key fields of research in the coming years.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/bias/Fig_biasworkflow.pdf}
    \caption{A schematic overview of the different biases that play a role during various stages of a machine learning workflow. Inspired by \cite{suresh2021framework}.}
    \label{fig:biasworkflow}
\end{figure*}

\subsection{Biases in machine learning workflows}
To understand how to identify and mitigate biases, it is important to consider how they emerge at various steps in the machine learning cycle \cite{suresh2021framework,hellstrom2020bias,friedler2019comparative}. Following the framework by Suresh and Guttag \cite{suresh2021framework}, six types of biases that emerge in a machine learning workflow are discussed.
\begin{enumerate}
\item \textbf{Historical bias}, which arises because field data captures phenomena that have already occurred in reality.  If the state of the world changes in the future, the model may not correctly capture those changes. For example, meteorological models trained on historical data may not perform well in the future if extreme events become more prominent \cite{lavell2012climate}. 
\item \textbf{Representation bias}, perhaps the most well-known type of bias when considering fairness. It concerns the way that the real world is sampled to generate the dataset used to train and evaluate the machine learning model. Representation bias occurs when certain parts of the population are under-represented in the sampling.
\item \textbf{Measurement bias}, induced as complex phenomena are defined in simpler concepts during dataset creation. For example, when predicting poverty through EO, poverty is often defined narrowly (e.g., percentage of the population below a defined poverty line) rather than considering broader aspects such as access to housing and sanitation \cite{lucci2018we}.
\item \textbf{Aggregation bias}, where subgroups of a population are aggregated into a single model instead of generating different models for distinct sub-groups.
\item \textbf{Evaluation bias}, stemming from the evaluation set used to assess model performance. Unequal representation of classes in the evaluation set, as well as the use of unsuitable performance metrics, can induce evaluation bias. For example, overall accuracy as an evaluation metric may be unsuitable for classification problems with unbalanced classes in remote sensing.
\item \textbf{Deployment bias}, arising from inappropriate interpretation and usage of the model results for decision-making. This can occur when model results are misinterpreted or applied in contexts for which they were not intended.
\end{enumerate}

\subsection{Auditing and mitigation strategies}
Two main streams of research can be considered in addressing biases in AI workflows: auditing for biases and implementing mitigation measures. 

Auditing a workflow for biases involves identifying causality, such as determining whether a sensitive attribute causes changes in the predicted variable, or examining statistical disparities between accuracy metrics of predictions for sub-groups defined by sensitive attributes \cite{castelnovo2022clarification}. For example, one might investigate whether building detection algorithms perform equally well in high-income and low-income neighborhoods of a city \cite{gevaert2023}. Calculating statistical disparities involves defining a sensitive attribute and determining which fairness metric is appropriate for the application. However, selecting a suitable fairness metric can be challenging as mathematical definitions of fairness may conflict \cite{barocas2019fairness,castelnovo2022clarification}. Interested readers are encouraged to explore resources on similarity-based metrics to understand the differences between metrics and how to select an appropriate one based on the application.

Bias mitigation can be applied at each step of the workflow individually. A recent review on data-centric learning in the field of GRS \cite{roscher2023data} highlights the importance of assessing dataset suitability throughout various stages of machine learning workflows. The review discusses how model bias can be addressed at each of these stages.


\subsection{Challenges and future directions}
There are several challenges specific to detecting biases in GRS applications. 

\subsubsection{Inference of Hidden Sensitive Attributes in ML Models} One challenge lies in defining the sensitive attributes. Societal concerns about which sub-groups should be treated fairly are often connected to demographic and socio-economic characteristics of individuals or groups. The UNESCO Recommendations \cite{unesco2021recommendation} describe fairness according to various categories such as age groups, cultural systems, language groups, persons with disabilities, girls and women, disadvantaged, marginalized and vulnerable populations, rural versus urban areas, and more. Similarly, the EU AI Act \cite{euaiact2021} is founded on Article 21 of the EU Charter of Fundamental Rights, which outlines non-discrimination related to sex, race, color, ethnic or social origin, genetic features, language, religion or belief, minority status, age and nationality, among others. Most of these characteristics are not included explicitly in the data utilized for GRS applications, with the exception perhaps of the urban-rural attribute mentioned by the UNESCO Recommendations. However, indirectly, these characteristics are often inferred. For example, there is extensive research on the identification of slums in satellite sensor imagery \cite{kuffer2016slums, mahabir2018critical}. Although the image does not contain information on poverty directly, the characteristics of the built-up environment have an indirect relation. Similarly, mobility data obtained through mobile phones may overrepresent higher income groups \cite{schlosser2021biases}. Therefore, despite not explicitly listing "sensitive" attributes in the data, geospatial and EO data are implicitly linked to these attributes. A significant challenge is to identify which sensitive attributes could be inferred from the data used to train and evaluate a machine learning model.

\subsubsection{Spatial Correlation Biases in GRS} A second challenge is that of spatial autocorrelation, which is specific to the manipulation of spatial data and is often overlooked when applying methods developed in computer vision directly to geospatial data. Karasiak et al. (2022) demonstrated how the spatial dependence between training and testing samples causes an overestimation of model accuracy \cite{karasiak2022spatial}. Other studies indicated how spatial autocorrelation plays a role in estimating the relations between air pollution and asthma \cite{park2022spatial} and in the estimation of ecosystem services \cite{shaikh2021accounting}. However, auditing for spatial correlation biases is underrepresented in the broader literature on Responsible AI in machine learning. It is expected that identifying and mitigating biases in models will be a particularly active direction of research in the fields of GRS. 

==> rspai_arxiv/3-ai-security.tex <==
\section{Secure AI in EO: Focusing on Defense Mechanisms, Uncertainty Modeling and Explainability}
\label{sec:security}
%%%%%%%%%%%%%%%%%%%%%%%%%% Possible Outline %%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition of the related terminologies.
% Literature review for AI security in remote sensing.
% Future perspectives (potential research directions and trends).

% length: around 2-3 pages
% num of ref: around 20-40 refs
%%%%%%%%%%%%%%%%%%%%%%%%%% General Suggestions from Pedram %%%%%%%%%%%%%%%%%%%%%%%%%% 
% Problem definition (with key equations if needed), its role in RS, its categories (with a bird’s eye view), a few examples for each category, and some nice figures or tables
%AI techniques have demonstrated considerable success across diverse geoscience and RS applications in recent decades. Despite their promising performance, concerns regarding the potential security threats posed by these AI algorithms have surfaced, as highlighted in studies like \cite{xu2023ai} and \cite{zhang2022artificial}. Particularly, the intricate modeling and complex parameters inherent in these AI techniques can significantly amplify the challenges associated with comprehending and explaining these black-box models. This, in turn, may escalate security risks observed in geoscience and RS applications across various domains. In response, %it becomes imperative for 
%AI techniques led to increased accuracy in GRS applications, but concerns about security threats have been raised \cite{xu2023ai}\cite{zhang2022artificial}. The intricate modelling and complex parameters of these AI methods pose challenges in understanding and explaining black-box models, potentially increasing security risks in various domains of GRS. For example, many real-time security cases regarding the usage of AI4EO reported in the past five years and reveal the vulnerability of current AI approaches, especially in high-risk EO missions, such as cyberattacks \cite{blasch2017big}, and data tampering problems \cite{xu2023integrity}. Researchers, therefore, are required to pinpoint the vulnerabilities within AI algorithms and devise corresponding security methods to increase the robustness of these models. This not only ensures increased accuracy but also fosters greater accountability in the context of geoscience and RS applications.


\begin{table*}[h]
\caption{Summary of the 3 AI security concerns including adversarial examples, uncertainty, and explainability.}
\label{table:summary_security}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{p{23mm}p{50mm}p{40mm}p{50mm}}
\specialrule{1pt}{0pt}{0pt} % thicker line
Security Concerns & Adversarial Examples                                                                 & Uncertainty                                                                 & Explainability                                                                                                   \\  \hline 
Sources           & Model and data-specific adversarial attacks                                          & Error and randomness in the training and testing data, and model parameters & Complexity arising from intricate structures of the \textit{black-box} models.                                              \\
Consequences      & Significantly reduces the performance of trained AI models                           & Inability to control the reliability of model results                       & Untrustworthiness and non-assessability of AI models due to the invisible working process of the \textit{black-box} models. \\
Defense methods   & Adversarial training, randomization, detection, and adversarial purification methods & Uncertainty quantification methods                                          & Explainable AI (XAI) approaches   \\                                              \specialrule{1pt}{0pt}{0pt} % thicker line                                  
\end{tabular}}
\end{table*}

In the context of EO, ensuring AI security is vital for upholding responsible AI principles and safeguarding against potential risks and vulnerabilities. EO systems rely increasingly on AI technologies for tasks ranging from image analysis and classification to predictive modeling. However, the integration of AI introduces security concerns such as data integrity threats, adversarial attacks on models, and privacy breaches. Addressing these challenges requires a comprehensive approach that considers both the technical aspects of AI security, such as explainable architectures and uncertainty modeling techniques, and ethical dimensions, including transparency, accountability and the protection of sensitive information. By incorporating AI security measures into the development and deployment of AI4EO systems, we can foster trust, reliability, and societal benefit while mitigating potential harms and ensuring that AI technologies contribute positively to environmental monitoring, disaster response, and sustainable development efforts. While aspects such as ethical dimensions, mitigating unfair biases, and preserving (geo)privacy are largely explained in Sections \ref{sec:unfair}, \ref{sec:privacy}, and \ref{sec:ethical}, we focus on uncertainty modeling, adversarial defenses, and explainability in this section.

\subsection{Security Hazards in AI Algorithms}\label{security-hazards}
Table \ref{table:summary_security} illustrates the primary concerns regarding AI security in GRS, encompassing adversarial attacks, the uncertainty of AI predictions, and the explainability of black-box models. These significant concerns will be addressed in this section. While this paper aims to emphasize concepts, we employ basic equations in this section to define AI security concerns. %In particular, the existence of adversarial attack samples with imperceptible perturbations against deep learning models can significantly degrade the performance of AI algorithms. Furthermore, the utilization of complex AI approaches with deeper architectures increases the difficulties of understanding and interpreting these black-box models. Additionally, the heterogeneity within the large-scale geoscience and RS data and the stochastic nature of the machine learning models can lead to uncertainty in the algorithms' predictions.

%\subsubsection{Adversarial Attacks}\label{attack}
\begin{figure}[ht!]
    \centering
    \includegraphics[scale=0.30]{figures/ai_security/figure1.pdf}
    \caption{Illustration of adversarial attack: a minor perturbation can fool the classifier into wrong predictions. \cite{yu2023universal}}
    \label{fig:papers}
\end{figure}
\subsubsection{Adversarial Examples}
%Adversarial examples for deep learning models have been discovered in various geoscience and RS tasks \cite{xu2020assessing}\cite{chen2021empirical} and have further motivated research on adversarial attacks against deep neural networks (DNNs). With a slightly imperceptible perturbation added to the data, the adversarial examples can easily fool the well-trained DNNs and cause significant performance loss even on state-of-the-art AI approaches. 
The identification of adversarial examples in AI4EO tasks \cite{xu2020assessing,chen2021empirical} has forced research into adversarial attacks on deep neural networks (DNNs). By introducing imperceptible perturbations to the data, these adversarial examples can deceive well-trained DNNs, leading to substantial performance degradation, even in state-of-the-art AI approaches like image classification and semantic segmentation \cite{xu2022universal}. Since the deep learning-based AI4EO methods minimize loss functions as an object to train the models, adversarial attacks employ the idea of maximizing the loss functions to find a perturbation to contaminate the clean samples, which can consequently fool well-trained AI4EO algorithms. As a result, this behavior severely threatens the responsibility of the current AI4EO approaches by making them predict incorrect results with high confidence. 

Adversarial attacks can appear virtually and physically when applying deep learning models.
On the one hand, the attackers can directly modify the applied remote sensing data before they are forwarded to the application models. For example, \citet{wu2023adversarial} demonstrated that the current end-to-end autonomous driving system could be easily broken by tempering the data with mild perturbations generated by white-box attacks. On the other hand, physical attack methods are more imperceptible since the adversarial perturbations are introduced during the remote sensing imaging process \cite{czaja2018adversarial}. \citet{zhang2022adversarial} explored the physical attack in real-world AI4EO applications by applying an adversarial patch attack on the multi-scale object detection for UAV remote sensing images.
As a corollary, responsible AI is required to mitigate the potential threats of these adversarial perturbations. Adversarial defense methods are desired that improve the reliability and response of the model, which are introduced in a later paragraph in this section.

% Taking image classification as an example, let $\mathcal{X} \to \mathcal{Y}$ represent a classifier mapping from the image space $\mathcal{X} \in \mathbb{R}^{d}$ to the label space $\mathcal{Y} \in \mathbb{R}^{K}$ with model parameters $\theta$, where $d$ and $K$ denote the number of pixels and categories, respectively. The common way to generate adversarial samples against the classifier is to find a perturbation $\delta \in \mathbb{R}^{d}$ that maximizes the loss function used for classification $\mathcal{L}$, ensuring $f(x+\delta)\neq y$, where $y$ is the correct predicted label of an image $x$. 


% Following this idea, the adversarial perturbation $\delta^{*}$ can be obtained with an optimisation equation as follows:
% \begin{equation}\label{adv_attack}
% 	\delta^{*} = \underset{B(x, \epsilon)}{\arg\max}\, \mathcal{L}(\theta, x + \delta, y),
% \end{equation}
% where $B(x, \epsilon)$ represents the allowed perturbation set and is defined as $B(x, \epsilon):=\{x + \delta \in \mathbb{R}^{d} \mid \lVert\delta\rVert_{p} \leq \epsilon\}$. Common values for $p$ are in the set $\{0, 1, 2, \infty\}$, and $\epsilon$ is typically set to a small value to ensure that perturbations remain imperceptible to the human eye. To solve Eq. (\ref{adv_attack}), various adversarial attack approaches have employed gradient-based methods \cite{jiang2021project,chen2021empirical}, which find the optimal adversarial perturbation by calculating the gradients of the loss function $\mathcal{L}_{ce}$. %One of the most commonly used methods is the Iterative Fast Gradient Sign Method (IFGSM) \cite{kurakin2016adversarial}. This method updates the adversarial perturbation in several iterations, as shown below:
%\begin{equation}
%	\delta^{t+1} = \alpha \cdot \text{sign}(\nabla_{x^{t}}\mathcal{L}(\theta, x^{t} + \delta, y)),
%\end{equation}
%where $t$ is the current step, $\alpha$ is the step size (usually smaller than $\epsilon$), $\text{sign}$ is the sign function, and $x^{t}$ denotes the adversarial sample generated in the $t$th iteration, where $x^{t} = x^{t-1} + \delta^{t}$.

\subsubsection{Uncertainty of the Model Predictions}\label{uncertain}
%Typically, geoscience and remote sensing data are commonly acquired from diverse platforms, resulting in a range of domain distributions. This diversity introduces uncertainty in model predictions when employing AI algorithms. Moreover, the stochastic nature inherent in machine learning models amplifies model uncertainty, posing a substantial challenge to the reliability of predictions. Hence, it is imperative to discern the presence of uncertainty and exert control over model outcomes. This becomes crucial in the development of more responsible geoscience and remote sensing AI models.
GRS data, often sourced from varied platforms, exhibit diverse domain distributions, introducing uncertainty in AI model predictions, as described in Section I. The stochastic nature of machine learning models further amplifies this uncertainty, posing a significant challenge to prediction reliability \cite{foody2002current}. Recognizing and managing uncertainty is vital for the development of responsible AI4EO models. The application of AI in GRS data involves distinct training and testing phases to optimize a mapping function $f_{\theta}: \mathcal{X}\to \mathcal{Y}$, where $\theta$ represents the initialized parameters. To this end, uncertainties may arise in the samples of training and testing datasets, as well as in the model parameters, categorized into data and model uncertainty \cite{dungan2002toward,persson2020characterizing}.

%In general, the application of AI in geoscience and RS data involves distinct training and testing phases, to optimize a mapping function $f_{\theta}: \mathcal{X}\to \mathcal{Y}$ as outlined in Section \ref{security-hazards}, where $\theta$ represents the initialized parameters. In the training phase, the model refines its parameters to $\hat{\theta}$ by minimizing errors in its predictions using a specified loss function. Subsequently, during the testing phase, samples from the testing dataset, denoted as $x^{*} \in \mathcal{X}^{*}$, are processed to generate predictions $y^{*} \in \mathcal{Y}^{*}$ using the trained model $f_{\hat{\theta}}$ for deployment. Throughout the aforementioned steps, uncertainties may arise in the training and testing datasets, as well as in the model parameters, categorized into data and model uncertainty.

%Data uncertainty encompasses the randomness and bias present in the data samples of both training and testing datasets. This uncertainty may arise from measurement errors in the raw data and a lack of domain knowledge bridging the training and testing datasets. Specifically, in understanding the uncertainty in the raw data collection stage, the Guide to the Expression of Uncertainty in Measurement (GUM) has been proposed. GUM characterizes uncertainty as an additive parameter associated with the measurement outcome, attributed to the measured raw Earth Observation (EO) data, i.e., $\mathcal{X}$ and $\mathcal{X}^{*}$. However, representing and directly estimating uncertainty in the measurement of raw data remains a challenging task. Additionally, the subset of ground truths in the training dataset, denoted as $\mathcal{Y}$, is often artificially labeled. This artificial labeling introduces uncertainty due to errors and discrete annotations of land surfaces.

Lack of domain knowledge is a prominent factor contributing to data uncertainty, arising from the disparate domain distribution observed between the training dataset $\mathcal{X}$ and the testing dataset $\mathcal{X}^{*}$. In remote sensing imaging, spectral features of observed data are closely tied to spatial and temporal conditions, such as solar illumination, season, and weather. Consequently, variations in these conditions can markedly influence imaging outcomes, resulting in heterogeneous data with diverse domain distributions, a phenomenon known as domain invariance \cite{tuia2016domain}. Regrettably, existing AI approaches struggle to make accurate predictions with a decision boundary that accounts for data exhibiting domain invariance, often referred to as domain shift \cite{tuia2021recent}. This poses a significant threat to model performance, particularly when faced with data uncertainty in testing samples during the model deployment stage. In attempts to mitigate domain shift issues, numerous studies in geoscience and remote sensing have proposed methods to adapt and extend the decision boundary of classification models to encompass unknown data in inference samples \cite{zhang2023cross,xu2022eyes}. However, these methods can only fine-tune models to a limited extent, and the data uncertainty associated with domain invariance cannot be eradicated entirely.
%%%==============================
In addition to data uncertainty, model uncertainty encompasses the errors and randomness inherent in the model parameters $\theta$, initialized and optimized during the model design and training processes. As researchers strive to develop advanced AI algorithms with cutting-edge performance and efficient training, diverse model architectures linked with optimization strategies have been devised for various GRS applications \cite{lin2021comparative}. However, determining the optimal model architecture and training hyperparameters remains challenging, introducing uncertainty into the trained model that can subsequently impact predictions, commonly referred to as model uncertainty \cite{doicu2021overview}.

%The complexity of model architectures can lead to challenges such as under- and over-fitting when mismatched with the volume of the training data. Simultaneously, the choice of training configurations, including loss functions and hyperparameters, directly controls the model fitting steps and cumulatively influences the final training quality. For instance, a training iteration using the widely adopted Stochastic Gradient Descent (SGD) optimizer can be defined as follows:
%\begin{equation}
%	\theta^{i+1} = \sum_{b=1}^{B} (\theta^{i} - \eta^{i}\nabla\mathcal{L}(\theta^{i}, x, y))/B,
%\end{equation}
%where $\mathcal{L}$ is the loss function, $\eta$ is the learning rate, and $B$ is the batch size. In this optimization function, the learning rate $\eta$ controls the amplitude of each step, while gradient descent determines the directions of the update. Employing a common mini-batch optimization strategy, the model is often trained with a batch of $B$ data samples. Due to the heterogeneity of the training data, each sample in the batch can be calculated into different optimization directions, contributing to an uncertain result in the update step. In conclusion, the judicious selection of optimization configurations becomes an uncertain aspect in the training of AI algorithms on geoscience and remote sensing data.

\subsubsection{Opacity of Black Box Models}\label{blackbox}

As high-performance computing technology advances, contemporary AI applications in geoscience and remote sensing studies explore models with deeper architectures and more complex parameters to enhance classification performance. However, the increased complexity raises challenges in understanding and interpreting the internal operational steps of these architectures, rendering the models akin to black boxes \cite{black2018model}. Compared with traditional machine learning approaches, the opacity of these black box models hinders the identification of hidden security hazards that can significantly impact classification, as well as the reasons for "wrong" predictions in real-world applications \cite{brendel2017decision}.
Moreover, the growing emphasis on data privacy and high confidentiality in many GRS tasks underscores the need for trustworthy AI models aligned with ethical and judicial requirements for both developers and users.

%In recent geoscience and RS studies, researchers have developed a series of complicated techniques, such as self-attention-based transformers \cite{zhang2022multilevel} and densely connected convolutional networks \cite{cai2021landslide}, which can accurately extract and process the meticulous deep representations of desired objects in images to achieve higher performance. Although these schemes achieved great success in various tasks, the amount of model parameters has exploded while the internal pathways between different modules in the DNNs have become more intricate. As a result, the black-box attribute of the modern DNNs makes it challenging to analyze and understand the principles of these networks. Therefore, it is crucial to develop AI models with enhanced explainability to fulfill the heightened responsibility of geoscience and remote sensing applications.

\subsection{Robust Modelling for AI Security}

In response to the identified security hazards outlined in the preceding section, researchers are working towards the development of more robust AI models, emphasizing enhanced responsibility for AI security. Several strategies are being employed, including adversarial defense, uncertainty quantification and explainable AI, to address challenges related to adversarial examples, data and model uncertainty, and black-box models, respectively.

\subsubsection{Adversarial Defense}

%Adversarial attacks pose a significant threat to DNNs, particularly in safety-critical geoscience and remote sensing applications. Consequently, it is essential to develop effective adversarial defense methods to enhance the resilience of deployed AI algorithms against adversarial samples. 
Common adversarial defense approaches include adversarial training, randomization, detection, and adversarial purification methods. Adversarial training methods aim to bolster the model's robustness against adversarial examples by incorporating them directly into the model training stage alongside normal training samples. For example, Goodfellow \cite{goodfellow2014explaining} proposed an empirical adversarial training scheme involving the inclusion of extra-generated Fast Gradient Sign Method (FGSM) attack adversarial samples. However, it is important to note that adversarial training methods may enhance the model's robustness against specific attack methods, yet vulnerabilities against adversarial examples of other types may persist.

Given that adversarial perturbations can be perceived as additive noise on adversarial examples, randomness methods introduce random components to enhance the model's robustness. For example, Cohen developed a randomized smoothing technique for adversarially robust classification involving the randomization of the input to the DNN to eliminate potential adversarial perturbations in the input samples \cite{sitawarin2022demystifying}. However, it is important to note that the performance of randomness methods depends greatly on the quality of the randomization process and can be affected significantly by both the lack of prior knowledge of attack types and theoretical explanations.

%In contrast to directly fine-tuning the model parameters of the target DNNs, detection methods focus on identifying the presence of adversarial examples and excluding them from normal test samples \cite{ai2021adversarial}. Typically, these methods incorporate an additional neural network-based detection module, such as a discriminator network, to determine whether a test sample contains adversarial perturbations. Although this reduces the detrimental impact of adversarial examples, the models may still struggle to generate correct predictions for these samples, which is unacceptable in certain data-driven applications. Furthermore, adversarial purification methods adopt a straightforward approach to defending DNNs by directly removing adversarial perturbations from samples using an additional purification network \cite{xu2022task}.

\subsubsection{Uncertainty Quantification}

%As discussed in Section \ref{uncertain}, data and model uncertainties are inherent and cannot be eradicated completely from AI applications in geoscience and remote sensing. 
To better comprehend and manage potential uncertainty, uncertainty quantification techniques have been proposed to assess the credibility of predictions.

In many GRS applications, classification results manifest as distributions of possibilities associated with object classes. These distributions are typically transformed by a softmax function at the final stage of the network. Grounded in the principles of Bayesian inference, the data uncertainty of an input sample $x^{*}$ can be described as a posterior distribution over the class label $y^{*}$ given a set of model parameters $\theta$. Similarly, the model uncertainty can be formalized as a posterior distribution given the training dataset $\mathcal{D}=(\mathcal{X},\mathcal{Y})$, as expressed by the equation:
\begin{equation}
	\mathcal{P}(y|x^{*},\mathcal{D})=\int  \underset{\mathrm{data}}{\underbrace{\mathcal{P}(y|x^{*},\theta)}}\ 
	\underset{\mathrm{model}}{\underbrace{\mathcal{P}(\theta|\mathcal{D})d\theta}}.
\end{equation}
Building upon this equation, various uncertainty quantification approaches aim to obtain an uncertainty distribution $\sigma^{*}$ of model predictions $y^{*}$ by marginalizing $\theta$. These methods fall into two broad categories: deterministic methods and Bayesian inference methods, differing in subcomponent model structures and error characteristics. In deterministic methods, the parameters of AI models are deterministic and remain fixed during the inference step, aligning with the common behavior of most developed AI models. In contrast, Bayesian inference methods employ the Bayesian learning strategy, leveraging the ability to seamlessly integrate scalability, expressiveness, and predictive performance of neural networks for uncertainty quantification \cite{ma2021corn,de2014uncertainty}. 

%In deterministic methods, the parameters of AI models are deterministic and remain fixed during the inference step, aligning with the common behaviour of most developed AI models. Generally, the outputs of the classification model, parametrised by $\theta^{*}$, already represent a distribution of possibilities over the classes processed by the softmax function, defined as follows:
%\begin{equation}
%	\mathcal{P}(y|x^{*};\theta^{*})=\frac{e^{z_{c}(x^{*})}}{\sum_{k=1}^{K}e^{z_{k}(x^{*})}},
%\end{equation}
%where $z_{k}(x^{*})\in \mathbb{R}$ denotes the possibility of the $k$-th class in predicting the input sample $x^{*}$. However, predictions from the softmax function often suffer from poor calibration due to insufficient characterization, leading to overconfidence in well-trained neural networks \cite{mozejko2018inhibited}. To address these issues, various approaches have employed Dirichlet prior networks to parameterize the distribution over a simplex \cite{gawlikowski2022advanced,yin2022quantifying}. These networks utilize Dirichlet prior distributions with tractable analytic properties, representing the density of predicted probabilities over categories. Consequently, data uncertainty can be quantified, taking into account domain distributions in Dirichlet distribution representations, by analyzing directly the logit magnitude of neural networks.

%In contrast, Bayesian inference methods employ the Bayesian learning strategy, leveraging the ability to seamlessly integrate scalability, expressiveness, and predictive performance of neural networks for uncertainty quantification \cite{ma2021corn,de2014uncertainty}. Specifically, Bayesian Neural Networks (BNNs) are employed to generate predictions as a probability distribution over the model parameters $\theta$, which can be utilized directly for uncertainty quantification. However, since the model parameters are integrated as a posterior distribution, approximation methods such as Monte Carlo methods are typically applied to facilitate the quantification process.

\subsubsection{Explainable AI}
In general, explainable AI (XAI) aims to provide an understanding of the pathways through which output decisions are made based on the parameters and activations of the trained models. To this end, many XAI approaches have been proposed for a comprehensive understanding of the model behavior to justify the individual feature attributions of a test sample $x \in \mathcal{X}$, which provides a powerful tool to examine incorrect predictions and inspect the potential threats of black-box models, especially in high-risk GRS applications \cite{hasanpour2022unboxing}. For example, \citet{ribeiro2016should} developed a Local Interpretable Model-agnostic Explanation (LIME) method to provide understandable representations for the predictions of black-box classifiers by highlighting attentive contiguous superpixels of the source image with positive weight towards a class, which benefits users in learning "how the model thinks" when classifying a specific image. Furthermore, the deep features of DNNs can also be processed into visualizations to observe how the training procedure works on specific tasks, as shown in Fig. \ref{fig:XAI}.
\begin{figure}[ht!]
    \centering
    \includegraphics[scale=0.20]{figures/ai_security/XAI.png}
    \label{fig:XAI}
    \caption{Heatmaps of UNet decoder block with different CAM-based XAI algorithms for the class of "buildings" in the semantic segmentation of an RS image. (source from \cite{gizzini2023extending}). Pixels that have a brighter color indicate a higher probability of being classified into the target class.}
\end{figure}
%In the literature, the XAI approaches designed for geoscience and RS applications are mainly developed as external analysis modules that extract local representations from model pathways to produce human-interpretable explanations for the AI models. For example, \citet{maddy2021miidaps} proposed an AI-based multi-instrument inversion and data assimilation preprocessing system (MIIDAPS-AI) for infrared and microwave polar and geostationary sounders and imagers, which can generate machine learning-based Jacobians to provide reliable explanations for the results. Furthermore, \citet{kakogeorgiou2021evaluating} demonstrated the applicability and explainability of XAI approaches in providing valuable insights for understanding the behaviors of black-box deep learning models applied to geoscience and RS datasets. Moreover, the Shapely Additive Explanation (SHAP) algorithm is employed to explain the predictions of multilayer perceptrons (MLPs) by analyzing the impact of each feature descriptor for post-earthquake building damage assessment \cite{lundberg2017unified}. %In particular, the XAI approach designed for this study provides further evidence for classification results (i.e., whether a building has collapsed or not) and, thus, increases the reliability of the AI models.

%Although the deep features of DNNs are usually considered to be highly abstract, some XAI approaches process them into visualizations to observe how the training procedure works on specific tasks, as shown in Fig. \ref{fig:XAI}. For example, \citet{xu2019beyond} incorporated Class Activation Mapping (CAM) techniques to calculate the contribution of each pixel to the predicted result by generating a heatmap for visual interpretation. In particular, this study found a high consistency between the deep feature maps from multiple layers and the object detection results by visualizing the response of activations of the neurons over different categories. Moreover, \citet{huang2021better} developed an encoder-classifier-reconstruction CAM (ECR-CAM) to improve visual interpretation of the more complex scenes contained in geoscience and RS data. Besides, \citet{xu2023txt2img} introduced XAI techniques into text-to-image generation tasks in geoscience and RS imagery to interpret the learned prototypes in text-image embeddings by visualizing 20 tokens involved in the basic components for image generation, such as different colors and texture patterns.

\subsection{Challenges and Future Perspectives}
%Although AI techniques have played an important role in many EO applications over the last decade, the potential security hazards should not be neglected and, thus, there exists the critical awareness of developing AI with more responsibility regarding their attributes of more robustness towards adversarial attacks, more reliability for the uncertainty of predictions, and more explainability and transparency for the common black-box AI models. However, the performance of existing security methods in geoscience and RS is still limited and needs to be increased due to the individual design of specific model architectures and the increasing complexity of geoscience and RS datasets. 
In this section, we discuss the future perspectives of AI security for EO tasks from three perspectives:

\subsubsection{The Game between Adversarial Attack and Defense towards EO Applications}
While adversarial examples have been identified widely in several EO applications, research on adversarial attacks and defense algorithms has been developed and raised the debate in game theory. On the one hand, the attackers have proposed more powerful attack algorithms to affect a wider range of DNNs applied in various EO missions, including scene classification and semantic segmentation. On the other hand, the defense group has also identified the emerging adversarial threats and tended to secure AI algorithms from more complex adversarial examples with frontier techniques, such as diffusion models \cite{yu2023universal}. In conclusion, the game between adversarial attack and defense algorithms has been started and extended to more subtopics in the AI4EO research field \cite{pal2020game}.

\subsubsection{Practical Uncertainty Analysis for AI4EO}
The uncertainty in both model and data towards AI4EO missions has been a critical obstacle for developing AI models with more reliability and responsibility. Although some uncertainty quantification methods have been seen in geoscience and RS studies, most of them were designed for dedicated models and are not adaptable to most of the existing AI4EO approaches. To this end, universal uncertainty analysis with greater capability to be applied in more typical DNNs should be developed for the AI4EO missions.

\subsubsection{XAI Schemes with more Understandable Interpretations}
Explainability is considered to be a significant attribute of modern AI4EO missions, which provides the opportunity for humans to learn the intrinsic process of the AI algorithms, security risks can be largely alleviated. However, current XAI methods designed for EO missions can only generate visualization interpretations, which are usually semantically misaligned and still too abstract to understand directly. Therefore, future XAI studies should focus on increasing the depth and accuracy of XAI results by introducing more constraints and optimization problems to explanations.



%Detailed information on these hazards are provides in the following contents.

==> rspai_arxiv/4-accountability.tex <==
\section{Accountability in AI4EO}
\label{sec:accountability}
%%%%%%%%%%%%%%%%%%%%%%%%%% Possible Outline %%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition of the related terminologies.
% Literature review for accountability in AI4EO.
% Future perspectives (potential research directions and trends).
  
% length: around 2-3 pages
% num of ref: around 20-40 refs
%%%%%%%%%%%%%%%%%%%%%%%%%% General Suggestions from Pedram %%%%%%%%%%%%%%%%%%%%%%%%%% 
% Problem definition (with key equations if needed), its role in RS, its categories (with a bird’s eye view), a few examples for each category, and some nice figures or tables

==> rspai_arxiv/5-privacy.tex <==
\section{Geo-Privacy and Privacy-preserving Measures}
\label{sec:privacy}
%%%%%%%%%%%%%%%%%%%%%%%%%% Possible Outline %%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition of the related terminologies.
% Literature review for (Geo)Privacy and Privacy-preserving Measures in remote sensing.
% Future perspectives (potential research directions and trends).
  
% length: around 2-3 pages
% num of ref: around 20-40 refs
%%%%%%%%%%%%%%%%%%%%%%%%%% General Suggestions from Pedram %%%%%%%%%%%%%%%%%%%%%%%%%% 
% Problem definition (with key equations if needed), its role in RS, its categories (with a bird’s eye view), a few examples for each category, and some nice figures or tables
%General introduction: definition and problem of privacy in Earth observation

Remotely sensed images and geospatial data offer unprecedented opportunities to monitor our planet and support spatial planning, management and decision-making. Nevertheless, as remote sensing technologies evolve, the need to balance the advantages of data-driven decision-making with the protection of individual privacy becomes paramount. The increasing resolution and quality of remotely sensed data, with their ability to capture detailed information about the Earth's surface and (directly or indirectly) the people living in those areas, raises concerns about the potential misuse of data and the accidental revelation of sensitive information \cite{HARRIS2021101422}. AI technologies allow the scale-up of geospatial applications, reducing analysis costs and subjectivity and, at the same time, magnifying the risk of exposing sensitive personal information.

Effectively addressing the above challenges requires thoughtful consideration of ethical principles, legal frameworks, and technological safeguards to ensure that the benefits of geospatial advances are realized without compromising individual privacy rights. Earlier research endeavors aimed at constructing a conceptual privacy framework; for example, \cite{finn2013seven} identified seven different concepts of privacy by examining distinct emerging technologies. 

\subsection{Privacy in UAV images}
In remote sensing, privacy concerns often arise when the resolution of an image is sufficiently fine to discern individuals' identities and expose personal details. This scenario commonly occurs during the analysis of images captured by Unmanned Aerial Vehicles (UAVs), potentially encroaching upon: (1) Location privacy, as individuals can be identified and tracked within UAV images. (2) Behavior privacy within private settings, free from external surveillance. (3) Space privacy, revealing details about secluded areas like backyards. (4) Association privacy, disclosing group memberships and affiliations. (5) Data and image privacy, involving individuals' control over images featuring their presence. 

Gevaert et al. \cite{gevaert2018evaluating} evaluated the societal impacts of using UAVs for informal settlement mapping through two case studies in Eastern Africa. The study stresses the importance of notifying citizens of the purpose of data collection, the rights to access, data processing, and distribution, especially when flying over marginalized communities. The absence of a cohesive policy framework governing such activities shifts a significant portion of responsibility onto industry self-regulation, potentially falling short of adequately safeguarding marginalized communities. Nevertheless, the existence of a ‘unified’ framework is challenged by the specific application of UAV image acquisition and the fact that the concept of sensitive information or privacy may vary among people, groups, and cultures. The study illustrates the importance of considering the local context regarding privacy issues.
Another example application with potentially privacy-related concerns is the use of UAV images in support of first responders in emergency situations (e.g., after an earthquake or other types of disasters). The authors in \citep{zhang2022training} developed a deep-learning network to detect victims in UAV images, which is trained to detect humans even in complex situations where body parts of the victims are partially covered by dust or debris. However, collecting a dataset for training such a network is challenging because of the sensitive nature of the data. Therefore, the authors proposed a framework to generate a harmonious composite of images for training. The framework first pastes images of body parts onto a debris background to generate composite victim images, then uses a deep harmonization network to make the composite images more harmonious.

\subsection{Mapping Sensitive Information}
Besides decimeter/centimetre-resolution UAV images, privacy concerns may also arise with satellite sensor images of various resolutions, especially when applied to map societal and socioeconomic features. Examples of sensitive applications include the mapping of informal settlements, slums,  deprived urban areas \cite{kuffer2018scope, kuffer2021spatial, persello2017deep} and refugee camps \cite{HASSAN2022103120}. The peril associated with disclosing sensitive information is evident in the "Mass Atrocity Remote Sensing" initiative, which sought to furnish forensic evidence of crimes against humanity through the analysis of satellite sensor imagery and other datasets. Nevertheless, researchers soon recognized that these data could also be exploited to identify and harm individuals and groups.
Publishing sensitive maps should always be done with care to prevent unintended consequences for local communities. In the case of informal settlements, being classified as living in such a neighborhood may result in social exclusion or even exposure to eviction (e.g., see the reports of forced evictions of 30,000 people from Nairobi’s largest slum, Kibera, in 2018 for building a new road \cite{bbc2018kenya}). Measures for privacy preservation typically include downgrading map spatial resolution (e.g., to cells of 100×100 m), aggregating data at the administrative unit level, and removing geo-location from datasets.

Another strategy to preserve household privacy is to apply jitter to geospatial point data (adding random noise to geocoordinates). The authors of \cite{chi2022microestimates} developed a comprehensive and openly accessible collection of microestimates detailing the distribution of relative poverty and wealth across 135 low- and middle-income countries (LMICs). They gathered data from Demographic and Health Surveys (DHSs) through traditional face-to-face surveys conducted with 1,457,315 distinct households residing in 66,819 villages spread across 56 different LMICs globally. The DHS data contain approximate GPS coordinates indicating the centroid of each surveyed village among the 66,819. However, to safeguard privacy, the precise geocoordinates are obfuscated, with a margin of error of up to 2 km in urban areas and up to 5 km in rural areas.

\subsection{Challenges and Future Perspectives}

A recent challenge is the increasing availability of satellite sensor images with sub-meter resolution up to 30 cm (e.g., WorldView-3, Pleiades NEO, Skysat) able to capture potentially sensitive information. The potential of such data for mapping and object detection should, therefore, be counterbalanced with privacy-preserving measures. Moreover, it is worth noting that privacy requirements may clash with open science principles, restricting the possibility of openly publishing and benchmarking datasets. 

Future investigations should develop strategies to openly share data for scientific advancements while preserving sensitive personal or group information. Such strategies are much needed in applications such as mapping deprived urban areas or victim detection, where further advances in the development of AI-based methods critically depend on the availability of large benchmark datasets, which are currently missing. 


%Considerations around group privacy, identity politics, and the security of data arise in this situation \cite{taylor2017safety}. Group privacy revolves around the consequences of data acquisition, processing, and utilization for members of a group, even if individual identities remain undisclosed. 


%Problems arise in applications such as:
%socioeconomic data,
%migration, refugee camps,
%example: Eyes on Darfur
%\cite{gordon2016monitoring}

%Mosaic effect - combining different datasets
%\cite{masinde2023group}

%Mitigation strategies:
%- Downsample map resolutions
%- NHS - household data with random noise added to locations %\cite{chi2022microestimates}

%\url{https://dataforgood.facebook.com/dfg/tools/relative-wealth-index#resources}

%google street view images 


==> rspai_arxiv/6-ethical.tex <==
\section{Maintaining Scientific Excellence, Open Data, and Guiding AI Usage Based on Ethical Principles in EO}
\label{sec:ethical}
%%%%%%%%%%%%%%%%%%%%%%%%%% Possible Outline %%%%%%%%%%%%%%%%%%%%%%%%%%
% Definition of the related terminologies.
% Literature review for Ethical Principles in remote sensing.
% Future perspectives (potential research directions and trends).
  
% length: around 2-3 pages
% num of ref: around 20-40 refs
%%%%%%%%%%%%%%%%%%%%%%%%%% General Suggestions from Pedram %%%%%%%%%%%%%%%%%%%%%%%%%% 
% Problem definition (with key equations if needed), its role in RS, its categories (with a bird’s eye view), a few examples for each category, and some nice figures or tables

The real-world character of AI4EO applications with downstream political, societal, and environmental impacts offers tremendous opportunities for positive change while simultaneously bearing the risk of negative impacts when not carefully designed and implemented \cite{hanson_garbage_2023, rolf_mission_2024, wagstaff_machine_2012}. Maintaining the highest scientific standards and making data and code openly accessible while complying with ethical principles are essential prerequisites to enhance the transparency of knowledge production, ensuring high reproducibility of scientific work and maximizing the societal, economic or environmental benefits of AI4EO research, development and applications \cite{hanson_garbage_2023}. Compliance with fundamental ethical principles is, thus, a major duty of the scientific community.  

A series of review papers laid out the relevant definitions and concepts of ethics in AI. For example, Jobin et al. (2019) \cite{jobin_global_2019} identified five broad categories from ethical guidelines in AI research: transparency, justice and fairness, non-maleficence, responsibility and privacy. With a focus on AI4EO, Kochupillai et al. (2022) \cite{kochupillai_earth_2022}, layed out six ethical dimensions: privacy, honesty, integrity, fairness, responsibility, and sustainability (for an overview on recent AI ethics categorizations, see Table 2 in \cite{kochupillai_earth_2022}). We here revisit the six categories proposed by \cite{kochupillai_earth_2022} focusing on aspects that transcend the themes of maintaining scientific excellence, open data, and guiding AI usage in AI4EO, that is, directly or indirectly relate to workflows, from defining objectives and research questions, data inputs and analysis outputs and their downstream impacts.  

\subsection{Privacy}\label{eth_privacy}

In the context of responsible AI4EO, we situate privacy concerns arising under the open data paradigm and with regard to (territorial) stigmatization. Open access to datasets and code is a core element of scientific reproducibility. Scientific excellence in AI4EO can, thus, only be achieved when the public dissemination of essential research data and code are made available to enable full reproducibility and robustness checks \cite{kedron_how_2022}. The scientific community has pushed for improving the Findability, Accessibility, Interoperability and Reuse of digital assets, which materialized in the FAIR-principles \cite{wilkinson_fair_2016}. Increasingly, however, the publication of geospatial data, including UAV or fine to very-fine-resolution satellite sensor imagery, labeled datasets, or the outputs of AI4EO workflows, may raise privacy concerns \cite{richardson_replication_2015}, see \ref{sec:privacy}). The FAIR-principles demand data to be free from use restrictions, fees or embargos, but legal, moral, or ethical reasons, such as safeguarding individual privacy, or endangered species, may justify deviation from these best practices on data accessibility \cite{kinkade_geoscience_2022}. However, detailed metadata should be made available enabling the discovery of such data and describe explicitly the conditions under which data access can be granted. 

Trade-offs between the benefits of open data and privacy concerns therefore need to be evaluated case-by-case to avoid privacy-violating or other ethically concerning impacts of public data dissemination. Besides the techniques to obscur geolocation information described above, a selective disclosure of data upon requests may be justified to avoid risks of data misuse. Additionally, purpose-specific data licensing may provide opportunities to avoid unintended use of datasets. One example for purpose-oriented data releases is Norway's International Climate and Forests Initiative (NICFI) Satellite Data Program, providing commercial satellite imagery covering the world´s tropics for non-commercial sustainability-centered applications (https://www.planet.com/nicfi/). 


Stigmatization may occur in cases where urban neighborhoods are categorized as slums \cite{kochupillai_conducting_2023, oluoch_crossing_2024}, or categorizations of crime rates or poverty levels adversely affect public perceptions of a community \cite{tang_predicting_2022}. The resulting territorial stigmatization may influence decision-making and negatively affect the local population. Similarly, stigmatization applies to AI4EO applications failing to consider the realities on the ground, for example, designed to expose illegal activities, such as deforestation, fire use, or mining activities, without knowledge about potential concessions to conduct the respective activity. Similarly, stigmatization may occur when global or broad-scale analyses fail to sufficiently consider local realities. For example, small-scale farming has been found to be responsible for 97\% of deforestation on the African continent \cite{branthomme_how_2023}, but regional dynamics such as the rapid emergence of medium-scale commercial farming operations \cite{jayne_changing_2022, wineman_relationship_2022}, the increasing role of export-oriented commodity crops such as cocoa, cashew and oil palm in deforestation \cite{masolele_mapping_2024}, and trade-offs between environmental degradation, food production, livelihoods and labor opportunities in semi-subsistence agriculture \cite{chiarella_balancing_2023,meyfroidt_trade-offs_2018} allow for a more nuanced perspective of such dynamics. As such, avoiding stigmatization of people, communities, or localities requires a high level of awareness of researchers in the design of research questions and label heuristics, as well as embedding scientific findings and their limitations in the realities of the region under investigation \cite{tulbure_regional_2022}. We highlight that cooperation with regionally knowledgeable partners in the early project design phase is an efficient way to avoid pitfalls of stigmatization in responsible AI4EO \cite{haelewaters_ten_2021}.
 
\subsection{Honesty}\label{eth_honesty}

Truthfulness and trustworthiness are inherent to scientific inquiry, but the current replication crisis undermines the credibility of science and, thus, hampers the societal uptake of scientific outputs. As a community producing knowledge with real-world impact, responsible AI4EO requires transparency, explainability, and data veracity \cite{hanson_garbage_2023}. 

In AI4EO, transparency not only requires thorough documentation and referencing of the datasets and workflows used but also that need to understand and clearly communicate ambiguities, potential biases, and errors, or conceptual limitations. In light of the ongoing democratization of EO data and workflows through cloud platforms, and accessible user interfaces, empowerment through access to EO data requires a thorough understanding of the limitations of EO data and workflows. Furthermore, transparency enables critical reflection of scientific findings. One example is a recent study linking the observed emerging abilities of LLMs (sudden, unexpected increases in performance) to study design choices made by researchers (e.g. evaluation metrics) \cite{schaeffer_are_2023}. 

Assuring explainability in AI4EO continues to be challenging, but is a prerequisite for early diagnostics regarding unwanted bias and sources of error. We strongly encourage the community to conduct  research on XAI, and incorporate it, wherever possible. Focusing research on explainable AI4EO will contribute to the recognition of EO data as a distinct modality in the AI community at large, by better understanding how AI models leverage the information contained in EO data \cite{rolf_mission_2024}. Greater explainability may also profit the emerging sub-field of self-supervised learning \cite{wang_self-supervised_2022}, and help to ensure oversight of (geographic) biases in AI4EO foundation models which claim high degrees of geographic generalization, but which are trained in selected world regions \cite{jakubik_foundation_2023}. Such biases are, for example, present in LLMs \cite{manvi_large_2024}, and may lead to error propagation to many downstream applications \cite{bommasani_opportunities_2021}. 

Data veracity in EO concerns both the imagery and the EO data pre-processing workflows used, as well as reference data / labels being in accordance with a (non-stigmatizing) heuristic defining the objects of interest. Using well-established and tested processing pipelines to assure the highest possible quality of EO data, for example, in terms of atmospheric correction \cite{doxani_atmospheric_2023}, but also regarding QA flags, including cloud masks for optical data \cite{skakun_cloud_2022}, is recommended to avoid downstream errors related to poor data quality. Labeling (the process of categorizing real-world phenomena into distinct classes or groups) is highly context-specific. Therefore, it requires regional expertise and knowledge, is ideally coordinated with local experts, and can be considered an iterative process in which exchange of knowledge from various disciplinary lenses is an effective means to reduce the risk of false categorizations or stigmatization \cite{tulbure_regional_2022}.

\subsection{Integrity}\label{eth_integrity}
Technical robustness and uncertainty reporting are key elements of integrity in AI4EO. Detailed documentation and reporting of the employed processing pipelines, including the respective processor version, enhances the reproducibility of AI4EO analyses. Detailed reporting of biases, errors, and uncertainty adds credibility and is detrimental to avoid erroneous use of datasets in downstream applications. Given the increasingly close interactions between the ML and EO communities, the maintenance and use of well-established evaluation standards particular to the EO domain, such as in reporting map accuracies and area estimates in categorical settings \cite{olofsson_good_5}, or for detecting trends in spatiotemporal data \cite{ives_statistical_2021} is key. 

In AI4EO research, a focus on single aggregate evaluation metrics (e.g. overall accuracy), as discussed in Section \ref{sec:unfair}, is insufficient, as often the detection of minority classes is most relevant in many AI4EO applications. Generally, and for imbalanced problems in particular, reporting area-adjusted class-specific user´s and producer´s accuracies from an independent and randomized sample must be preferred over simplistic one-dimensional statistics. Similarly, class area estimates are to be derived from reference samples rather than pixel counting in maps with non-random error distribution. For continuous targets (e.g. reflectance, biomass, crop yields, canopy height), reporting multiple error metrics and assessing them across the entire value range reveals heteroskedasticity and can inform downstream users of potential pitfalls when using a product \cite{frantz_understanding_2023}.

\subsection{Fairness}\label{eth_fairness}

Fairness here refers to avoiding bias, and to respecting all aspects of diversity and sociocultural differences, ultimately creating standards based on principles related to fairness. Bias may relate to all stages of AI4EO analyses, beginning with defining a research question, through the workflow itself, and ending with the manifold downstream impacts related to interpreting the results - as laid out in \ref{sec:unfair}. We will not delve deeper into the broader ethical framework discussed elsewhere \cite{kochupillai_earth_2022, xu_ai_2023}. Instead, we focus on core needs, before, during and after setting up an AI4EO workflow.

Before setting up an AI4EO workflow, we may consider opportunities to invite potential stakeholders of anticipated outcomes to participate in co-creating the research agenda  \cite{brandsen_definitions_2018}. Stakeholders typically include different institutions across all levels, from village heads in an area of interest to the United Nations or the World Bank. Stakeholders may also be citizens who are acquainted with the topic or the area of interest, ideally (but not mandatory) being engaged in related citizen-science opportunities \cite{verburg_land_2015}, such as data sampling or field-based mapping evaluation \cite{fritz_geo-wiki_5, schepaschenko_development_6}. Citizens and institutions acquainted with the research questions will help to mitigate bias in the project design phase.

During workflow creation, interpretable AI, as discussed in Section \ref{sec:security}, should support paving the way towards optimizing workflows and avoiding downstream misinterpretations \cite{gevaert_explainable_2022, rudin_stop_2019}. Interpretable AI also allows tuning algorithms and workflows based on the scientists’ and non-science stakeholders’ expertise \cite{graziani_global_2023}. Non-scientists thereby provide consultancy to EO scientists to overcome the different biases mentioned in Section \ref{sec:unfair} during the workflow implementation and roll-out, including historical, representation, measurement, aggregation and evaluation bias (compare \ref{sec:unfair} A). Next to training data creation, providing sufficient and independent evaluation data for accuracy assessment is both of core importance and often one of the most challenging tasks (see also \ref{eth_integrity}).

Implicitly, avoiding workflow-related bias is also tightly connected to recognizing deployment bias.  Deployment bias relates to the inappropriate interpretation of results after the data analysis, which is often related to downstream decision-makers. This underlines the importance of co-creation and co-production to minimize and mitigate deployment bias early on. In other words, confronting stakeholders with results created in the scientific “ivory tower” without engaging with them in the design and production phase regularly creates unsatisfactory results for those affected or supposed to build their decision-making processes on AI4EO outcomes. 

Deployment bias also points directly to the need to respect diversity and sociocultural differences. For example, we need to recognize different ethnic or religious communities, as well as AI4EO experts compared to non-expert stakeholders to avoid mis-interpretations or disrespectful outcomes of AI4EO workflows. Typical examples are the mapping of slums or of agricultural practices in the Global South \cite{kochupillai_conducting_2023, nakalembe_considerations_2023}. Many studies on related research questions need to integrate stakeholders early on in AI4EO to include the necessary expertise to create meaningful results, specifically across large areas of interest, where diverse and multicultural stakeholders are needed. AI4EO workflows also rarely consider resource restrictions in the Global South - regarding the “data desert”, limited processing resources, or limited financial backup, e.g. for implementing cloud computing or using HPC or supercomputing facilities \cite{stahl_ethics_2023}. In other words, cooperation at “eye level” is needed to embed AI4EO in the proper sociocultural context, specifically when solving SDG-related questions and global change issues in the Global South \cite{gevaert_explainable_2022, haelewaters_ten_2021}. In conclusion, we create win-win situations when joining the forces of stakeholders "on the ground" (deliberately including stakeholders across scales from local dwellers to global institutions, depending on the research questions to be tackled) with AI4EO experts.

\subsection{Responsibility}\label{eth_responsibility}
The need for interdisciplinary and regional collaboration related to domain knowledge across the entire workflow of AI4EO and unwanted outcomes or interpretations were tackled in the section on “Fairness”. We, therefore, here focus on handling the distinctness of EO data well \cite{rolf_mission_2024}. 

It has been argued that the AI/ML community urgently needs to recognize the distinct features of satellite-based EO data and to “move out of the comfort zone” of applying AI methods established in other domains without improved adaptation to EO or satellite data machine learning (SatML, \cite{rolf_mission_2024}). The reasons are manifold as, for example:
\begin{itemize}
    \item Satellite data is rarely “analysis-ready data” (ARD) \cite{frantz_forcelandsat_2019}), requiring state-of-the-art preprocessing to represent the same values for the same features in different images, i.e., to avoid pseudo-variance.
    
    \item Spatial autocorrelation according to Tobler’s first law of geography \cite{miller_toblers_2004} is rarely used to improve AI4EO, even less so newer concepts like Partitioned Autoregressive Time-Series (PARTS) that consider both spatial and temporal autocorrelation in a congruent fashion \cite{ives_statistical_2021}

    \item Satellite data provide a wide range of spatial resolutions (from very-fine-resolution to pixels of several $\mathrm{km}^{2}$) and extend across all scales to be observed (from local, fine-scale objects in urban environments to global phenomena). Both very diverse spatial detail and multi-scale research ask for adapted solutions.
    
    \item Different temporal resolutions, i.e., data densities over time, represent the same land surface differently. In other words, change analyses over years or decades are far from trivial, and need contextualization \cite{frantz_revisiting_2022, frantz_understanding_2023}. This is even more important when phenology is considered and specific temporal windows across the seasons are crucial to identify the relevant phenomena, e.g. different crop types, land use intensities or tree species separable only at certain phenological stages \cite{blickensdorfer_national_2024,lobert_deep_2023,schwieder_mapping_2022}.

    \item Most AI algorithms for image analyses were developed on three-band red-green-blue (RGB) imagery, often based on VHR drone data. Today’s multi- to hyperspectral satellite data ask for more sophisticated approaches to detect not just the obvious, but the relevant. This is aggravated by more spectral detail in radiometric data beyond 8-bit and even more by using virtual constellations \cite{wulder_virtual_12}, ranging from optical over radar to LiDAR data.

    \item Sparse labeling problems occur with increasing areas of interest enabled by AI4EO. More severe problems are inherited by biased samples across larger regions or non-trivial features to be sampled from existing data or the imagery itself \cite{rufin_taking_2023, wang_unlocking_2022}.
\end{itemize}

While all these aspects are relevant for any EO analysis framework, opportunities have increased rapidly with AI4EO (e.g., regarding the size of areas of interest that can be handled). Along with these are the related risks and potential awareness deficits. Many, if not the majority of, AI4EO studies focused on comparably small use cases in the past to develop or apply algorithms. However, the roll-out to real-world problems, for example, at the national, continental or even global scale, requires ubiquitous algorithms that can handle much more diverse feature spaces (over time). There is indeed a lack of upscaling studies demonstrating the suitability of most algorithms for tackling real-world problems \cite{rolf_mission_2024, tuia_toward_2021, tuia_artificial_2023}.

\subsection{Sustainability}\label{eth_sustainability}
Since 2015, the United Nations has set an ambitious agenda related to the Sustainable Development Goals (SDG), aiming to improve social, economic and environmental conditions globally by 2030 \cite{un_transforming_2015, Persello_2022}, with a wealth of implications for AI and also specifically for AI4EO \cite{stahl_ethics_2023}. Here, we take the broadest possible standpoint, including the intrinsic sustainability of AI4EO workflows and the external impacts for all three SDG dimensions. Given that AI at large offers the potential for both positive and negative impacts across all SDGs, with a majority on social sustainability \cite{vinuesa_role_2020}, AI4EO has a similar potential for both positive and negative impacts.

Focusing on environmental sustainability, EO is data- and energy-hungry, thereby creating immense $\mathrm{CO}_{2}$ emissions. This footprint relates to the entire lifecycle of EO engineering, science and outcomes, including but not being limited to building, launching and running satellite missions, data creation and curation, data storage and data analysis workflows - the data-related aspects being core for AI4EO \cite{wilkinson_environmental_2024}.

Zooming in on economic and social SDG, the FAIR principles are highly relevant: We thematized avoiding “helicopter research” already in \ref{eth_fairness} \cite{haelewaters_ten_2021}. Offering inclusiveness is non-trivial to deliver, as many EO scientists and companies, specifically in the Global South, do not have access to powerful cloud computing or HPC services or to GPU-equipped high-performance workstations. Even if access to online services may become available through dedicated programs or international cooperations, proper education and training for the next generation of AI4EO scientists is of utmost importance \cite{stahl_ethics_2023}.

The outcomes from AI4EO research may greatly support improvements along the lines of the UN SDGs \cite{Persello_2022, vinuesa_role_2020} - but may also lead to ill-posed conclusions. Such conclusions can, in the worst case, create an existential economic threat (e.g., if loans or insurance are not provided based on AI4EO-derived indicators \cite{benami_uniting_2021}). Also, local stakeholders including indigenous people, who may not even be aware of governments’ decision making processes, are regularly impacted, though. Last but not least, AI4EO may be in the “wrong hands”; for example, used by autocrats, dictators, or criminals to suppress or threaten specifically environmental and social SDGs. The most disturbing examples of this are ubiquitous AI4EO-supported surveillance and warfare. 

